Origins and Nature of Macroeconomic Instability in Vector Autoregressions

For a general class of dynamic and stochastic structural models, we show that (i) non-linearity in economic dynamics is a necessary and sufficient condition for time-varying parameters (TVPs) in the reduced-form VARMA process followed by observables, and (ii) all parameters' time-variation is driven by the same, typically few sources of stochasticity: the structural shocks. Our results call into question the common interpretation that TVPs are due to "structural instabilities". Motivated by our theoretical analysis, we model a set of macroeconomic and financial variables as a TVP-VAR with a factor-structure in TVPs. This reveals that most instabilities are driven by a few factors, which comove strongly with measures of macroeconomic uncertainty and the contribution of finance to real economic activity, commonly emphasized as important sources of non-linearities in macroeconomics. Furthermore, our model yields improved forecasts relative to the standard TVP-VAR where TVPs evolve as independent random walks.

==> FcstTables/2CRPS_Model_1_Prior_3_Lag_2_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\clearpage
\includegraphics[scale=1]{./Model_1_Prior_3_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1/2CRPS_Model_1_Prior_3_Lag_2_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.eps}
\begin{flushleft}
{\raggedright Notes: RMSFE for Data 1, Prior 3, Lag 2, Neval 98, Sampling mode 1, Difference mode 1 and Factor mode 1.}
\end{flushleft}
\label{fig:2CRPSModel1Prior3Lag2FcstNeval98SamplingMode1DifMode1FacMode1}


==> FcstTables/2CRPS_Model_1_Prior_3_Lag_5_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\clearpage
\includegraphics[scale=1]{./Model_1_Prior_3_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1/2CRPS_Model_1_Prior_3_Lag_5_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.eps}
\begin{flushleft}
{\raggedright Notes: RMSFE for Data 1, Prior 3, Lag 5, Neval 98, Sampling mode 1, Difference mode 1 and Factor mode 1.}
\end{flushleft}
\label{fig:2CRPSModel1Prior3Lag5FcstNeval98SamplingMode1DifMode1FacMode1}


==> FcstTables/2FI_Horizon_1_Model_1_Prior_3_Lag_2_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\clearpage
\includegraphics[scale=1]{./Model_1_Prior_3_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1/2FI_Horizon_1_Model_1_Prior_3_Lag_2_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.eps}
\begin{flushleft}
{\raggedright Notes: Posterior $68\%$ for Horizon 1, Data 1, Prior 3, Lag 2, Neval 98, Sampling mode 1, Difference mode 1 and Factor mode 1.}
\end{flushleft}
\label{fig:2FIHorizon1CRPSModel1Prior3Lag2FcstNeval98SamplingMode1DifMode1FacMode1}


==> FcstTables/2FI_Horizon_1_Model_1_Prior_3_Lag_5_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\clearpage
\includegraphics[scale=1]{./Model_1_Prior_3_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1/2FI_Horizon_1_Model_1_Prior_3_Lag_5_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.eps}
\begin{flushleft}
{\raggedright Notes: Posterior $68\%$ for Horizon 1, Data 1, Prior 3, Lag 5, Neval 98, Sampling mode 1, Difference mode 1 and Factor mode 1.}
\end{flushleft}
\label{fig:2FIHorizon1CRPSModel1Prior3Lag5FcstNeval98SamplingMode1DifMode1FacMode1}


==> FcstTables/2FI_Horizon_8_Model_1_Prior_3_Lag_2_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\clearpage
\includegraphics[scale=1]{./Model_1_Prior_3_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1/2FI_Horizon_8_Model_1_Prior_3_Lag_2_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.eps}
\begin{flushleft}
{\raggedright Notes: Posterior $68\%$ for Horizon 8, Data 1, Prior 3, Lag 2, Neval 98, Sampling mode 1, Difference mode 1 and Factor mode 1.}
\end{flushleft}
\label{fig:2FIHorizon8CRPSModel1Prior3Lag2FcstNeval98SamplingMode1DifMode1FacMode1}


==> FcstTables/2FI_Horizon_8_Model_1_Prior_3_Lag_5_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\clearpage
\includegraphics[scale=1]{./Model_1_Prior_3_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1/2FI_Horizon_8_Model_1_Prior_3_Lag_5_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.eps}
\begin{flushleft}
{\raggedright Notes: Posterior $68\%$ for Horizon 8, Data 1, Prior 3, Lag 5, Neval 98, Sampling mode 1, Difference mode 1 and Factor mode 1.}
\end{flushleft}
\label{fig:2FIHorizon8CRPSModel1Prior3Lag5FcstNeval98SamplingMode1DifMode1FacMode1}


==> FcstTables/2PIT_Horizon_1_Model_1_Prior_3_Lag_2_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\includegraphics[scale=1]{./Model_1_Prior_3_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1/PIT_Horizon_1_Model_1_Prior_3_Lag_2_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.eps}
\begin{flushleft}
{\raggedright Notes: RMSFE for Horizon 1, Data 1, Prior 3, Lag 2, Neval 98, Sampling mode 1, Difference mode 1 and Factor mode 1.}
\end{flushleft}
\label{fig:PITHorizon1CRPSModel1Prior3Lag2FcstNeval98SamplingMode1DifMode1FacMode1}


==> FcstTables/2PIT_Horizon_1_Model_1_Prior_3_Lag_5_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\includegraphics[scale=1]{./Model_1_Prior_3_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1/PIT_Horizon_1_Model_1_Prior_3_Lag_5_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.eps}
\begin{flushleft}
{\raggedright Notes: RMSFE for Horizon 1, Data 1, Prior 3, Lag 5, Neval 98, Sampling mode 1, Difference mode 1 and Factor mode 1.}
\end{flushleft}
\label{fig:PITHorizon1CRPSModel1Prior3Lag5FcstNeval98SamplingMode1DifMode1FacMode1}


==> FcstTables/2PIT_Horizon_8_Model_1_Prior_3_Lag_2_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\includegraphics[scale=1]{./Model_1_Prior_3_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1/PIT_Horizon_8_Model_1_Prior_3_Lag_2_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.eps}
\begin{flushleft}
{\raggedright Notes: RMSFE for Horizon 8, Data 1, Prior 3, Lag 2, Neval 98, Sampling mode 1, Difference mode 1 and Factor mode 1.}
\end{flushleft}
\label{fig:PITHorizon8CRPSModel1Prior3Lag2FcstNeval98SamplingMode1DifMode1FacMode1}


==> FcstTables/2PIT_Horizon_8_Model_1_Prior_3_Lag_5_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\includegraphics[scale=1]{./Model_1_Prior_3_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1/PIT_Horizon_8_Model_1_Prior_3_Lag_5_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.eps}
\begin{flushleft}
{\raggedright Notes: RMSFE for Horizon 8, Data 1, Prior 3, Lag 5, Neval 98, Sampling mode 1, Difference mode 1 and Factor mode 1.}
\end{flushleft}
\label{fig:PITHorizon8CRPSModel1Prior3Lag5FcstNeval98SamplingMode1DifMode1FacMode1}


==> FcstTables/Paper2TableInFeval_Model_1_Prior_3_Lag_1_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[!t]\centering
\caption{$68\%$ Interval forecast evaluation at lag 1 (Coverage and length).}
\label{fig:InFevalModel1Prior3Lag1FcstNeval98SamplingMode1DifMode1FacMode1}
\begin{center}
\begin{tabular}{lcc|cc|cc|cc}
\hline\hline
\textbf{Model} & \multicolumn{2}{c}{\textbf{1Q}}  & \multicolumn{2}{c}{\textbf{2Q}}  & \multicolumn{2}{c}{\textbf{4Q}}  & \multicolumn{2}{c}{\textbf{8Q}} \\ 
\hline
\multicolumn{9}{c}{\textbf{Real GDP}} \\ 
\hline
TVP-VAR-SV & $0.68$  & $[1.13]$ &	$0.68$ & $[1.21]$ &	$0.77^{\ast}$ & $[1.34]$ &	$0.76$  & $[1.60]$ \\ 
GF-TVP-VAR-SV & $0.66$  & $[1.15]$ &	$0.65$ & $[1.21]$ &	$0.63$ & $[1.29]$ &	$0.67$  & $[1.47]$ \\ 
CF-TVP-VAR-SV & $0.69$  & $[1.14]$ &	$0.68$ & $[1.20]$ &	$0.68$ & $[1.27]$ &	$0.69$  & $[1.46]$ \\ 
\hline
\multicolumn{9}{c}{\textbf{Inflation}} \\ 
\hline
TVP-VAR-SV & $0.74$  & $[0.46]$ &	$0.78^{\ast}$ & $[0.54]$ &	$0.80^{\ast\ast}$ & $[0.65]$ &	$0.85^{\ast\ast\ast}$  & $[0.84]$ \\ 
GF-TVP-VAR-SV & $0.74$  & $[0.47]$ &	$0.74$ & $[0.55]$ &	$0.80^{\ast\ast}$ & $[0.66]$ &	$0.84^{\ast\ast\ast}$  & $[0.85]$ \\ 
CF-TVP-VAR-SV & $0.80^{\ast\ast\ast}$  & $[0.46]$ &	$0.77$ & $[0.54]$ &	$0.81^{\ast}$ & $[0.64]$ &	$0.84^{\ast\ast\ast}$  & $[0.81]$ \\ 
\hline
\multicolumn{9}{c}{\textbf{FFR}} \\ 
\hline
TVP-VAR-SV & $0.67$  & $[0.84]$ &	$0.63$ & $[1.50]$ &	$0.61$ & $[2.73]$ &	$0.66$  & $[5.01]$ \\ 
GF-TVP-VAR-SV & $0.66$  & $[0.85]$ &	$0.65$ & $[1.52]$ &	$0.60$ & $[2.72]$ &	$0.68$  & $[4.80]$ \\ 
CF-TVP-VAR-SV & $0.72$  & $[0.84]$ &	$0.65$ & $[1.50]$ &	$0.66$ & $[2.68]$ &	$0.65$  & $[4.68]$ \\ 
\hline
\multicolumn{9}{c}{\textbf{Credit Spread}} \\ 
\hline
TVP-VAR-SV & $0.67$  & $[0.46]$ &	$0.61$ & $[0.71]$ &	$0.70$ & $[1.10]$ &	$0.76$  & $[1.68]$ \\ 
GF-TVP-VAR-SV & $0.64$  & $[0.46]$ &	$0.62$ & $[0.71]$ &	$0.67$ & $[1.07]$ &	$0.62$  & $[1.56]$ \\ 
CF-TVP-VAR-SV & $0.63$  & $[0.40]$ &	$0.61$ & $[0.62]$ &	$0.61$ & $[0.97]$ &	$0.65$  & $[1.48]$ \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: to be added}
\end{flushleft}
\end{table}


==> FcstTables/Paper2TableInFeval_Model_1_Prior_3_Lag_3_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[!t]\centering
\caption{$68\%$ Interval forecast evaluation at lag 3 (Coverage and length).}
\label{fig:InFevalModel1Prior3Lag3FcstNeval98SamplingMode1DifMode1FacMode1}
\begin{center}
\begin{tabular}{lcc|cc|cc|cc}
\hline\hline
\textbf{Model} & \multicolumn{2}{c}{\textbf{1Q}}  & \multicolumn{2}{c}{\textbf{2Q}}  & \multicolumn{2}{c}{\textbf{4Q}}  & \multicolumn{2}{c}{\textbf{8Q}} \\ 
\hline
\multicolumn{9}{c}{\textbf{Real GDP}} \\ 
\hline
TVP-VAR-SV & $0.70$  & $[1.22]$ &	$0.72$ & $[1.31]$ &	$0.74$ & $[1.50]$ &	$0.82^{\ast\ast}$  & $[1.77]$ \\ 
GF-TVP-VAR-SV & $0.68$  & $[1.22]$ &	$0.71$ & $[1.30]$ &	$0.73$ & $[1.48]$ &	$0.81^{\ast\ast}$  & $[1.73]$ \\ 
CF-TVP-VAR-SV & $0.68$  & $[1.18]$ &	$0.71$ & $[1.25]$ &	$0.72$ & $[1.44]$ &	$0.81^{\ast\ast}$  & $[1.69]$ \\ 
\hline
\multicolumn{9}{c}{\textbf{Inflation}} \\ 
\hline
TVP-VAR-SV & $0.79^{\ast\ast}$  & $[0.43]$ &	$0.73$ & $[0.48]$ &	$0.83^{\ast\ast\ast}$ & $[0.63]$ &	$0.87^{\ast\ast\ast}$  & $[0.86]$ \\ 
GF-TVP-VAR-SV & $0.80^{\ast\ast\ast}$  & $[0.43]$ &	$0.73$ & $[0.48]$ &	$0.83^{\ast\ast\ast}$ & $[0.63]$ &	$0.89^{\ast\ast\ast}$  & $[0.85]$ \\ 
CF-TVP-VAR-SV & $0.78^{\ast\ast}$  & $[0.44]$ &	$0.73$ & $[0.49]$ &	$0.83^{\ast\ast\ast}$ & $[0.64]$ &	$0.88^{\ast\ast\ast}$  & $[0.85]$ \\ 
\hline
\multicolumn{9}{c}{\textbf{FFR}} \\ 
\hline
TVP-VAR-SV & $0.68$  & $[0.75]$ &	$0.71$ & $[1.56]$ &	$0.65$ & $[2.89]$ &	$0.65$  & $[4.72]$ \\ 
GF-TVP-VAR-SV & $0.70$  & $[0.75]$ &	$0.71$ & $[1.57]$ &	$0.63$ & $[2.89]$ &	$0.66$  & $[4.71]$ \\ 
CF-TVP-VAR-SV & $0.76^{\ast}$  & $[0.80]$ &	$0.73$ & $[1.61]$ &	$0.66$ & $[2.86]$ &	$0.66$  & $[4.61]$ \\ 
\hline
\multicolumn{9}{c}{\textbf{Credit Spread}} \\ 
\hline
TVP-VAR-SV & $0.67$  & $[0.47]$ &	$0.65$ & $[0.74]$ &	$0.65$ & $[1.07]$ &	$0.71$  & $[1.55]$ \\ 
GF-TVP-VAR-SV & $0.68$  & $[0.47]$ &	$0.64$ & $[0.74]$ &	$0.63$ & $[1.06]$ &	$0.70$  & $[1.53]$ \\ 
CF-TVP-VAR-SV & $0.65$  & $[0.43]$ &	$0.63$ & $[0.68]$ &	$0.61$ & $[0.98]$ &	$0.65$  & $[1.45]$ \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: to be added}
\end{flushleft}
\end{table}


==> FcstTables/Paper2TableInFeval_Model_1_Prior_3_Lag_4_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[!t]\centering
\caption{$68\%$ Interval forecast evaluation at lag 4 (Coverage and length).}
\label{fig:InFevalModel1Prior3Lag4FcstNeval98SamplingMode1DifMode1FacMode1}
\begin{center}
\begin{tabular}{lcc|cc|cc|cc}
\hline\hline
\textbf{Model} & \multicolumn{2}{c}{\textbf{1Q}}  & \multicolumn{2}{c}{\textbf{2Q}}  & \multicolumn{2}{c}{\textbf{4Q}}  & \multicolumn{2}{c}{\textbf{8Q}} \\ 
\hline
\multicolumn{9}{c}{\textbf{Real GDP}} \\ 
\hline
TVP-VAR-SV & $0.72$  & $[1.33]$ &	$0.73$ & $[1.51]$ &	$0.81^{\ast\ast\ast}$ & $[1.86]$ &	$0.90^{\ast\ast\ast}$  & $[2.56]$ \\ 
GF-TVP-VAR-SV & $0.60$  & $[1.30]$ &	$0.70$ & $[1.42]$ &	$0.80^{\ast\ast}$ & $[1.71]$ &	$0.89^{\ast\ast\ast}$  & $[2.26]$ \\ 
CF-TVP-VAR-SV & $0.56^{\ast\ast}$  & $[1.19]$ &	$0.66$ & $[1.29]$ &	$0.78^{\ast\ast}$ & $[1.57]$ &	$0.90^{\ast\ast\ast}$  & $[2.10]$ \\ 
\hline
\multicolumn{9}{c}{\textbf{Inflation}} \\ 
\hline
TVP-VAR-SV & $0.76^{\ast}$  & $[0.47]$ &	$0.78^{\ast}$ & $[0.54]$ &	$0.86^{\ast\ast\ast}$ & $[0.66]$ &	$0.88^{\ast\ast\ast}$  & $[1.01]$ \\ 
GF-TVP-VAR-SV & $0.79^{\ast\ast}$  & $[0.46]$ &	$0.79^{\ast\ast}$ & $[0.51]$ &	$0.86^{\ast\ast\ast}$ & $[0.63]$ &	$0.88^{\ast\ast\ast}$  & $[0.93]$ \\ 
CF-TVP-VAR-SV & $0.80^{\ast\ast\ast}$  & $[0.45]$ &	$0.79^{\ast\ast}$ & $[0.49]$ &	$0.85^{\ast\ast\ast}$ & $[0.60]$ &	$0.88^{\ast\ast\ast}$  & $[0.89]$ \\ 
\hline
\multicolumn{9}{c}{\textbf{FFR}} \\ 
\hline
TVP-VAR-SV & $0.76^{\ast}$  & $[0.78]$ &	$0.71$ & $[1.68]$ &	$0.76$ & $[3.20]$ &	$0.69$  & $[5.57]$ \\ 
GF-TVP-VAR-SV & $0.69$  & $[0.78]$ &	$0.66$ & $[1.68]$ &	$0.65$ & $[3.14]$ &	$0.64$  & $[5.30]$ \\ 
CF-TVP-VAR-SV & $0.73$  & $[0.83]$ &	$0.69$ & $[1.69]$ &	$0.62$ & $[3.00]$ &	$0.62$  & $[5.04]$ \\ 
\hline
\multicolumn{9}{c}{\textbf{Credit Spread}} \\ 
\hline
TVP-VAR-SV & $0.70$  & $[0.50]$ &	$0.66$ & $[0.82]$ &	$0.71$ & $[1.21]$ &	$0.84^{\ast\ast\ast}$  & $[1.90]$ \\ 
GF-TVP-VAR-SV & $0.68$  & $[0.50]$ &	$0.63$ & $[0.79]$ &	$0.67$ & $[1.15]$ &	$0.71$  & $[1.71]$ \\ 
CF-TVP-VAR-SV & $0.68$  & $[0.46]$ &	$0.62$ & $[0.73]$ &	$0.63$ & $[1.05]$ &	$0.67$  & $[1.58]$ \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: to be added}
\end{flushleft}
\end{table}


==> FcstTables/PaperTableInFeval_Model_1_Prior_3_Lag_1_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[h!]\centering
\caption{$68\%$ Interval forecast evaluation at lag 1 (Coverage and length).}
\begin{center}
\begin{tabular}{lcc|cc|cc|cc}
\hline\hline
Model & \multicolumn{2}{c}{h=1Q}  & \multicolumn{2}{c}{h=2Q}  & \multicolumn{2}{c}{h=4Q}  & \multicolumn{2}{c}{h=8Q} \\ 
\hline
\multicolumn{9}{c}{Real GDP} \\ 
\hline
TVP-VAR-SV & 0.68^{\ast\ast\ast} & [1.13] &	0.68^{\ast\ast\ast} & [1.21] &	0.77^{\ast\ast\ast} & [1.34] &	0.76^{\ast\ast\ast} & [1.60] \\ 
Model 1 & 0.66^{\ast\ast\ast} & [1.15] &	0.65^{\ast\ast\ast} & [1.21] &	0.63^{\ast\ast\ast} & [1.29] &	0.67^{\ast\ast\ast} & [1.47] \\ 
Model 2 & 0.66^{\ast\ast\ast} & [1.25] &	0.61^{\ast\ast\ast} & [1.31] &	0.57^{\ast\ast\ast} & [1.38] &	0.64^{\ast\ast\ast} & [1.54] \\ 
Model 3 & 0.69^{\ast\ast\ast} & [1.14] &	0.68^{\ast\ast\ast} & [1.20] &	0.68^{\ast\ast\ast} & [1.27] &	0.69^{\ast\ast\ast} & [1.46] \\ 
Model 4 & 0.64^{\ast\ast\ast} & [1.19] &	0.60^{\ast\ast\ast} & [1.24] &	0.58^{\ast\ast\ast} & [1.31] &	0.61^{\ast\ast\ast} & [1.48] \\ 
\hline
\multicolumn{9}{c}{Inflation} \\ 
\hline
TVP-VAR-SV & 0.74^{\ast\ast\ast} & [0.46] &	0.78^{\ast\ast\ast} & [0.54] &	0.80^{\ast\ast\ast} & [0.65] &	0.85^{\ast\ast\ast} & [0.84] \\ 
Model 1 & 0.74^{\ast\ast\ast} & [0.47] &	0.74^{\ast\ast\ast} & [0.55] &	0.80^{\ast\ast\ast} & [0.66] &	0.84^{\ast\ast\ast} & [0.85] \\ 
Model 2 & 0.77^{\ast\ast\ast} & [0.52] &	0.79^{\ast\ast\ast} & [0.62] &	0.79^{\ast\ast\ast} & [0.74] &	0.86^{\ast\ast\ast} & [0.93] \\ 
Model 3 & 0.80^{\ast\ast\ast} & [0.46] &	0.77^{\ast\ast\ast} & [0.54] &	0.81^{\ast\ast\ast} & [0.64] &	0.84^{\ast\ast\ast} & [0.81] \\ 
Model 4 & 0.78^{\ast\ast\ast} & [0.47] &	0.77^{\ast\ast\ast} & [0.56] &	0.80^{\ast\ast\ast} & [0.67] &	0.88^{\ast\ast\ast} & [0.84] \\ 
\hline
\multicolumn{9}{c}{FFR} \\ 
\hline
TVP-VAR-SV & 0.67^{\ast\ast\ast} & [0.84] &	0.63^{\ast\ast\ast} & [1.50] &	0.61^{\ast\ast\ast} & [2.73] &	0.66^{\ast\ast\ast} & [5.01] \\ 
Model 1 & 0.66^{\ast\ast\ast} & [0.85] &	0.65^{\ast\ast\ast} & [1.52] &	0.60^{\ast\ast\ast} & [2.72] &	0.68^{\ast\ast\ast} & [4.80] \\ 
Model 2 & 0.69^{\ast\ast\ast} & [0.91] &	0.66^{\ast\ast\ast} & [1.62] &	0.64^{\ast\ast\ast} & [2.93] &	0.68^{\ast\ast\ast} & [5.17] \\ 
Model 3 & 0.72^{\ast\ast\ast} & [0.84] &	0.65^{\ast\ast\ast} & [1.50] &	0.66^{\ast\ast\ast} & [2.68] &	0.65^{\ast\ast\ast} & [4.68] \\ 
Model 4 & 0.68^{\ast\ast\ast} & [0.86] &	0.67^{\ast\ast\ast} & [1.55] &	0.65^{\ast\ast\ast} & [2.81] &	0.68^{\ast\ast\ast} & [4.90] \\ 
\hline
\multicolumn{9}{c}{Credit Spread} \\ 
\hline
TVP-VAR-SV & 0.67^{\ast\ast\ast} & [0.46] &	0.61^{\ast\ast\ast} & [0.71] &	0.70^{\ast\ast\ast} & [1.10] &	0.76^{\ast\ast\ast} & [1.68] \\ 
Model 1 & 0.64^{\ast\ast\ast} & [0.46] &	0.62^{\ast\ast\ast} & [0.71] &	0.67^{\ast\ast\ast} & [1.07] &	0.62^{\ast\ast\ast} & [1.56] \\ 
Model 2 & 0.66^{\ast\ast\ast} & [0.47] &	0.62^{\ast\ast\ast} & [0.73] &	0.64^{\ast\ast\ast} & [1.11] &	0.59^{\ast\ast\ast} & [1.61] \\ 
Model 3 & 0.63^{\ast\ast\ast} & [0.40] &	0.61^{\ast\ast\ast} & [0.62] &	0.61^{\ast\ast\ast} & [0.97] &	0.65^{\ast\ast\ast} & [1.48] \\ 
Model 4 & 0.63^{\ast\ast\ast} & [0.40] &	0.60^{\ast\ast\ast} & [0.63] &	0.58^{\ast\ast\ast} & [0.99] &	0.61^{\ast\ast\ast} & [1.50] \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: to be added}
\end{flushleft}
\label{fig:InFevalModel1Prior3Lag1FcstNeval98SamplingMode1DifMode1FacMode1}
\end{table}


==> FcstTables/PaperTableInFeval_Model_1_Prior_3_Lag_2_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[h!]\centering
\caption{$68\%$ Interval forecast evaluation at lag 2 (Coverage and length).}
\begin{center}
\begin{tabular}{lcc|cc|cc|cc}
\hline\hline
Model & \multicolumn{2}{c}{h=1Q}  & \multicolumn{2}{c}{h=2Q}  & \multicolumn{2}{c}{h=4Q}  & \multicolumn{2}{c}{h=8Q} \\ 
\hline
\multicolumn{9}{c}{Real GDP} \\ 
\hline
TVP-VAR-SV & 0.68^{\ast\ast\ast} & [1.18] &	0.66^{\ast\ast\ast} & [1.26] &	0.79^{\ast\ast\ast} & [1.41] &	0.82^{\ast\ast\ast} & [1.65] \\ 
Model 1 & 0.66^{\ast\ast\ast} & [1.19] &	0.66^{\ast\ast\ast} & [1.26] &	0.72^{\ast\ast\ast} & [1.39] &	0.81^{\ast\ast\ast} & [1.61] \\ 
Model 2 & 0.66^{\ast\ast\ast} & [1.28] &	0.66^{\ast\ast\ast} & [1.37] &	0.69^{\ast\ast\ast} & [1.51] &	0.80^{\ast\ast\ast} & [1.70] \\ 
Model 3 & 0.71^{\ast\ast\ast} & [1.19] &	0.67^{\ast\ast\ast} & [1.24] &	0.70^{\ast\ast\ast} & [1.38] &	0.83^{\ast\ast\ast} & [1.58] \\ 
Model 4 & 0.67^{\ast\ast\ast} & [1.26] &	0.65^{\ast\ast\ast} & [1.32] &	0.68^{\ast\ast\ast} & [1.46] &	0.81^{\ast\ast\ast} & [1.65] \\ 
\hline
\multicolumn{9}{c}{Inflation} \\ 
\hline
TVP-VAR-SV & 0.78^{\ast\ast\ast} & [0.44] &	0.71^{\ast\ast\ast} & [0.50] &	0.82^{\ast\ast\ast} & [0.63] &	0.83^{\ast\ast\ast} & [0.82] \\ 
Model 1 & 0.77^{\ast\ast\ast} & [0.45] &	0.69^{\ast\ast\ast} & [0.50] &	0.79^{\ast\ast\ast} & [0.63] &	0.81^{\ast\ast\ast} & [0.82] \\ 
Model 2 & 0.78^{\ast\ast\ast} & [0.47] &	0.72^{\ast\ast\ast} & [0.53] &	0.83^{\ast\ast\ast} & [0.69] &	0.89^{\ast\ast\ast} & [0.90] \\ 
Model 3 & 0.77^{\ast\ast\ast} & [0.45] &	0.76^{\ast\ast\ast} & [0.51] &	0.83^{\ast\ast\ast} & [0.64] &	0.83^{\ast\ast\ast} & [0.82] \\ 
Model 4 & 0.76^{\ast\ast\ast} & [0.46] &	0.77^{\ast\ast\ast} & [0.53] &	0.85^{\ast\ast\ast} & [0.68] &	0.87^{\ast\ast\ast} & [0.88] \\ 
\hline
\multicolumn{9}{c}{FFR} \\ 
\hline
TVP-VAR-SV & 0.69^{\ast\ast\ast} & [0.76] &	0.70^{\ast\ast\ast} & [1.54] &	0.69^{\ast\ast\ast} & [2.92] &	0.70^{\ast\ast\ast} & [4.75] \\ 
Model 1 & 0.71^{\ast\ast\ast} & [0.76] &	0.71^{\ast\ast\ast} & [1.54] &	0.67^{\ast\ast\ast} & [2.91] &	0.67^{\ast\ast\ast} & [4.73] \\ 
Model 2 & 0.70^{\ast\ast\ast} & [0.77] &	0.72^{\ast\ast\ast} & [1.57] &	0.68^{\ast\ast\ast} & [3.03] &	0.66^{\ast\ast\ast} & [5.02] \\ 
Model 3 & 0.73^{\ast\ast\ast} & [0.81] &	0.76^{\ast\ast\ast} & [1.57] &	0.67^{\ast\ast\ast} & [2.88] &	0.65^{\ast\ast\ast} & [4.63] \\ 
Model 4 & 0.77^{\ast\ast\ast} & [0.79] &	0.74^{\ast\ast\ast} & [1.58] &	0.63^{\ast\ast\ast} & [2.96] &	0.65^{\ast\ast\ast} & [4.90] \\ 
\hline
\multicolumn{9}{c}{Credit Spread} \\ 
\hline
TVP-VAR-SV & 0.67^{\ast\ast\ast} & [0.46] &	0.60^{\ast\ast\ast} & [0.73] &	0.66^{\ast\ast\ast} & [1.09] &	0.69^{\ast\ast\ast} & [1.59] \\ 
Model 1 & 0.69^{\ast\ast\ast} & [0.46] &	0.61^{\ast\ast\ast} & [0.72] &	0.65^{\ast\ast\ast} & [1.09] &	0.69^{\ast\ast\ast} & [1.56] \\ 
Model 2 & 0.67^{\ast\ast\ast} & [0.47] &	0.61^{\ast\ast\ast} & [0.74] &	0.67^{\ast\ast\ast} & [1.12] &	0.67^{\ast\ast\ast} & [1.61] \\ 
Model 3 & 0.66^{\ast\ast\ast} & [0.42] &	0.62^{\ast\ast\ast} & [0.66] &	0.60^{\ast\ast\ast} & [1.00] &	0.66^{\ast\ast\ast} & [1.47] \\ 
Model 4 & 0.66^{\ast\ast\ast} & [0.43] &	0.61^{\ast\ast\ast} & [0.67] &	0.60^{\ast\ast\ast} & [1.03] &	0.65^{\ast\ast\ast} & [1.52] \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: to be added}
\end{flushleft}
\label{fig:InFevalModel1Prior3Lag2FcstNeval98SamplingMode1DifMode1FacMode1}
\end{table}


==> FcstTables/PaperTableInFeval_Model_1_Prior_3_Lag_3_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[h!]\centering
\caption{$68\%$ Interval forecast evaluation at lag 3 (Coverage and length).}
\begin{center}
\begin{tabular}{lcc|cc|cc|cc}
\hline\hline
Model & \multicolumn{2}{c}{h=1Q}  & \multicolumn{2}{c}{h=2Q}  & \multicolumn{2}{c}{h=4Q}  & \multicolumn{2}{c}{h=8Q} \\ 
\hline
\multicolumn{9}{c}{Real GDP} \\ 
\hline
TVP-VAR-SV & 0.70^{\ast\ast\ast} & [1.22] &	0.72^{\ast\ast\ast} & [1.31] &	0.74^{\ast\ast\ast} & [1.50] &	0.82^{\ast\ast\ast} & [1.77] \\ 
Model 1 & 0.68^{\ast\ast\ast} & [1.22] &	0.71^{\ast\ast\ast} & [1.30] &	0.73^{\ast\ast\ast} & [1.48] &	0.81^{\ast\ast\ast} & [1.73] \\ 
Model 2 & 0.72^{\ast\ast\ast} & [1.30] &	0.70^{\ast\ast\ast} & [1.40] &	0.72^{\ast\ast\ast} & [1.59] &	0.80^{\ast\ast\ast} & [1.82] \\ 
Model 3 & 0.68^{\ast\ast\ast} & [1.18] &	0.71^{\ast\ast\ast} & [1.25] &	0.72^{\ast\ast\ast} & [1.44] &	0.81^{\ast\ast\ast} & [1.69] \\ 
Model 4 & 0.70^{\ast\ast\ast} & [1.26] &	0.68^{\ast\ast\ast} & [1.35] &	0.73^{\ast\ast\ast} & [1.54] &	0.83^{\ast\ast\ast} & [1.77] \\ 
\hline
\multicolumn{9}{c}{Inflation} \\ 
\hline
TVP-VAR-SV & 0.79^{\ast\ast\ast} & [0.43] &	0.73^{\ast\ast\ast} & [0.48] &	0.83^{\ast\ast\ast} & [0.63] &	0.87^{\ast\ast\ast} & [0.86] \\ 
Model 1 & 0.80^{\ast\ast\ast} & [0.43] &	0.73^{\ast\ast\ast} & [0.48] &	0.83^{\ast\ast\ast} & [0.63] &	0.89^{\ast\ast\ast} & [0.85] \\ 
Model 2 & 0.79^{\ast\ast\ast} & [0.45] &	0.73^{\ast\ast\ast} & [0.51] &	0.85^{\ast\ast\ast} & [0.67] &	0.91^{\ast\ast} & [0.93] \\ 
Model 3 & 0.78^{\ast\ast\ast} & [0.44] &	0.73^{\ast\ast\ast} & [0.49] &	0.83^{\ast\ast\ast} & [0.64] &	0.88^{\ast\ast\ast} & [0.85] \\ 
Model 4 & 0.78^{\ast\ast\ast} & [0.45] &	0.76^{\ast\ast\ast} & [0.51] &	0.86^{\ast\ast\ast} & [0.68] &	0.92^{\ast\ast} & [0.92] \\ 
\hline
\multicolumn{9}{c}{FFR} \\ 
\hline
TVP-VAR-SV & 0.68^{\ast\ast\ast} & [0.75] &	0.71^{\ast\ast\ast} & [1.56] &	0.65^{\ast\ast\ast} & [2.89] &	0.65^{\ast\ast\ast} & [4.72] \\ 
Model 1 & 0.70^{\ast\ast\ast} & [0.75] &	0.71^{\ast\ast\ast} & [1.57] &	0.63^{\ast\ast\ast} & [2.89] &	0.66^{\ast\ast\ast} & [4.71] \\ 
Model 2 & 0.70^{\ast\ast\ast} & [0.76] &	0.70^{\ast\ast\ast} & [1.60] &	0.63^{\ast\ast\ast} & [3.02] &	0.65^{\ast\ast\ast} & [5.05] \\ 
Model 3 & 0.76^{\ast\ast\ast} & [0.80] &	0.73^{\ast\ast\ast} & [1.61] &	0.66^{\ast\ast\ast} & [2.86] &	0.66^{\ast\ast\ast} & [4.61] \\ 
Model 4 & 0.76^{\ast\ast\ast} & [0.80] &	0.69^{\ast\ast\ast} & [1.64] &	0.68^{\ast\ast\ast} & [2.98] &	0.65^{\ast\ast\ast} & [4.93] \\ 
\hline
\multicolumn{9}{c}{Credit Spread} \\ 
\hline
TVP-VAR-SV & 0.67^{\ast\ast\ast} & [0.47] &	0.65^{\ast\ast\ast} & [0.74] &	0.65^{\ast\ast\ast} & [1.07] &	0.71^{\ast\ast\ast} & [1.55] \\ 
Model 1 & 0.68^{\ast\ast\ast} & [0.47] &	0.64^{\ast\ast\ast} & [0.74] &	0.63^{\ast\ast\ast} & [1.06] &	0.70^{\ast\ast\ast} & [1.53] \\ 
Model 2 & 0.67^{\ast\ast\ast} & [0.48] &	0.65^{\ast\ast\ast} & [0.76] &	0.64^{\ast\ast\ast} & [1.10] &	0.68^{\ast\ast\ast} & [1.59] \\ 
Model 3 & 0.65^{\ast\ast\ast} & [0.43] &	0.63^{\ast\ast\ast} & [0.68] &	0.61^{\ast\ast\ast} & [0.98] &	0.65^{\ast\ast\ast} & [1.45] \\ 
Model 4 & 0.66^{\ast\ast\ast} & [0.44] &	0.64^{\ast\ast\ast} & [0.70] &	0.58^{\ast\ast\ast} & [1.03] &	0.63^{\ast\ast\ast} & [1.51] \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: to be added}
\end{flushleft}
\label{fig:InFevalModel1Prior3Lag3FcstNeval98SamplingMode1DifMode1FacMode1}
\end{table}


==> FcstTables/PaperTableInFeval_Model_1_Prior_3_Lag_4_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[h!]\centering
\caption{$68\%$ Interval forecast evaluation at lag 4 (Coverage and length).}
\begin{center}
\begin{tabular}{lcc|cc|cc|cc}
\hline\hline
Model & \multicolumn{2}{c}{h=1Q}  & \multicolumn{2}{c}{h=2Q}  & \multicolumn{2}{c}{h=4Q}  & \multicolumn{2}{c}{h=8Q} \\ 
\hline
\multicolumn{9}{c}{Real GDP} \\ 
\hline
TVP-VAR-SV & 0.72^{\ast\ast\ast} & [1.33] &	0.73^{\ast\ast\ast} & [1.51] &	0.81^{\ast\ast\ast} & [1.86] &	0.90^{\ast\ast} & [2.56] \\ 
Model 1 & 0.60^{\ast\ast\ast} & [1.30] &	0.70^{\ast\ast\ast} & [1.42] &	0.80^{\ast\ast\ast} & [1.71] &	0.89^{\ast\ast} & [2.26] \\ 
Model 2 & 0.63^{\ast\ast\ast} & [1.96] &	0.66^{\ast\ast\ast} & [1.94] &	0.77^{\ast\ast\ast} & [2.11] &	0.89^{\ast\ast} & [2.58] \\ 
Model 3 & 0.56^{\ast\ast\ast} & [1.19] &	0.66^{\ast\ast\ast} & [1.29] &	0.78^{\ast\ast\ast} & [1.57] &	0.90^{\ast\ast} & [2.10] \\ 
Model 4 & 0.50^{\ast\ast\ast} & [1.86] &	0.58^{\ast\ast\ast} & [1.81] &	0.66^{\ast\ast\ast} & [1.97] &	0.88^{\ast\ast\ast} & [2.43] \\ 
\hline
\multicolumn{9}{c}{Inflation} \\ 
\hline
TVP-VAR-SV & 0.76^{\ast\ast\ast} & [0.47] &	0.78^{\ast\ast\ast} & [0.54] &	0.86^{\ast\ast\ast} & [0.66] &	0.88^{\ast\ast} & [1.01] \\ 
Model 1 & 0.79^{\ast\ast\ast} & [0.46] &	0.79^{\ast\ast\ast} & [0.51] &	0.86^{\ast\ast\ast} & [0.63] &	0.88^{\ast\ast\ast} & [0.93] \\ 
Model 2 & 0.86^{\ast\ast\ast} & [0.63] &	0.87^{\ast\ast\ast} & [0.70] &	0.91^{\ast\ast\ast} & [0.87] &	0.97^{\ast} & [1.31] \\ 
Model 3 & 0.80^{\ast\ast\ast} & [0.45] &	0.79^{\ast\ast\ast} & [0.49] &	0.85^{\ast\ast\ast} & [0.60] &	0.88^{\ast\ast\ast} & [0.89] \\ 
Model 4 & 0.85^{\ast\ast\ast} & [0.62] &	0.88^{\ast\ast\ast} & [0.69] &	0.88^{\ast\ast\ast} & [0.85] &	0.97 & [1.27] \\ 
\hline
\multicolumn{9}{c}{FFR} \\ 
\hline
TVP-VAR-SV & 0.76^{\ast\ast\ast} & [0.78] &	0.71^{\ast\ast\ast} & [1.68] &	0.76^{\ast\ast\ast} & [3.20] &	0.69^{\ast\ast\ast} & [5.57] \\ 
Model 1 & 0.69^{\ast\ast\ast} & [0.78] &	0.66^{\ast\ast\ast} & [1.68] &	0.65^{\ast\ast\ast} & [3.14] &	0.64^{\ast\ast\ast} & [5.30] \\ 
Model 2 & 0.73^{\ast\ast\ast} & [0.97] &	0.66^{\ast\ast\ast} & [2.21] &	0.65^{\ast\ast\ast} & [4.41] &	0.67^{\ast\ast\ast} & [7.45] \\ 
Model 3 & 0.73^{\ast\ast\ast} & [0.83] &	0.69^{\ast\ast\ast} & [1.69] &	0.62^{\ast\ast\ast} & [3.00] &	0.62^{\ast\ast\ast} & [5.04] \\ 
Model 4 & 0.69^{\ast\ast\ast} & [1.00] &	0.64^{\ast\ast\ast} & [2.21] &	0.60^{\ast\ast\ast} & [4.29] &	0.59^{\ast\ast\ast} & [7.20] \\ 
\hline
\multicolumn{9}{c}{Credit Spread} \\ 
\hline
TVP-VAR-SV & 0.70^{\ast\ast\ast} & [0.50] &	0.66^{\ast\ast\ast} & [0.82] &	0.71^{\ast\ast\ast} & [1.21] &	0.84^{\ast\ast\ast} & [1.90] \\ 
Model 1 & 0.68^{\ast\ast\ast} & [0.50] &	0.63^{\ast\ast\ast} & [0.79] &	0.67^{\ast\ast\ast} & [1.15] &	0.71^{\ast\ast\ast} & [1.71] \\ 
Model 2 & 0.70^{\ast\ast\ast} & [0.59] &	0.68^{\ast\ast\ast} & [1.00] &	0.62^{\ast\ast\ast} & [1.46] &	0.68^{\ast\ast\ast} & [2.09] \\ 
Model 3 & 0.68^{\ast\ast\ast} & [0.46] &	0.62^{\ast\ast\ast} & [0.73] &	0.63^{\ast\ast\ast} & [1.05] &	0.67^{\ast\ast\ast} & [1.58] \\ 
Model 4 & 0.63^{\ast\ast\ast} & [0.55] &	0.58^{\ast\ast\ast} & [0.92] &	0.52^{\ast\ast\ast} & [1.36] &	0.62^{\ast\ast\ast} & [1.96] \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: to be added}
\end{flushleft}
\label{fig:InFevalModel1Prior3Lag4FcstNeval98SamplingMode1DifMode1FacMode1}
\end{table}


==> FcstTables/PaperTableInFeval_Model_1_Prior_3_Lag_5_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[h!]\centering
\caption{$68\%$ Interval forecast evaluation at lag 5 (Coverage and length).}
\begin{center}
\begin{tabular}{lcc|cc|cc|cc}
\hline\hline
Model & \multicolumn{2}{c}{h=1Q}  & \multicolumn{2}{c}{h=2Q}  & \multicolumn{2}{c}{h=4Q}  & \multicolumn{2}{c}{h=8Q} \\ 
\hline
\multicolumn{9}{c}{Real GDP} \\ 
\hline
TVP-VAR-SV & 0.78^{\ast\ast\ast} & [2.01] &	0.87^{\ast\ast\ast} & [2.35] &	0.95^{\ast} & [3.24] &	0.99 & [5.54] \\ 
Model 1 & 0.77^{\ast\ast\ast} & [1.87] &	0.83^{\ast\ast\ast} & [2.02] &	0.93^{\ast\ast} & [2.69] &	0.97 & [4.31] \\ 
Model 2 & 0.83^{\ast\ast\ast} & [3.08] &	0.88^{\ast\ast\ast} & [2.77] &	0.93^{\ast\ast} & [3.36] &	0.97 & [5.01] \\ 
Model 3 & 0.71^{\ast\ast\ast} & [1.78] &	0.80^{\ast\ast\ast} & [1.93] &	0.92^{\ast\ast} & [2.57] &	0.96 & [4.15] \\ 
Model 4 & 0.72^{\ast\ast\ast} & [2.92] &	0.80^{\ast\ast\ast} & [2.62] &	0.88^{\ast\ast\ast} & [3.14] &	0.97 & [4.62] \\ 
\hline
\multicolumn{9}{c}{Inflation} \\ 
\hline
TVP-VAR-SV & 0.82^{\ast\ast\ast} & [0.66] &	0.83^{\ast\ast\ast} & [0.78] &	0.93^{\ast\ast} & [1.08] &	0.98 & [1.99] \\ 
Model 1 & 0.83^{\ast\ast\ast} & [0.62] &	0.91^{\ast\ast\ast} & [0.69] &	0.91^{\ast\ast\ast} & [0.94] &	0.98 & [1.62] \\ 
Model 2 & 0.91^{\ast\ast\ast} & [0.92] &	0.96^{\ast\ast} & [0.95] &	0.96^{\ast} & [1.27] &	0.99 & [2.08] \\ 
Model 3 & 0.82^{\ast\ast\ast} & [0.59] &	0.86^{\ast\ast\ast} & [0.66] &	0.90^{\ast\ast} & [0.90] &	0.98 & [1.59] \\ 
Model 4 & 0.91^{\ast\ast\ast} & [0.88] &	0.95^{\ast\ast} & [0.91] &	0.94^{\ast\ast} & [1.20] &	0.99 & [1.98] \\ 
\hline
\multicolumn{9}{c}{FFR} \\ 
\hline
TVP-VAR-SV & 0.80^{\ast\ast\ast} & [0.91] &	0.80^{\ast\ast\ast} & [2.00] &	0.82^{\ast\ast\ast} & [3.98] &	0.81^{\ast\ast\ast} & [7.51] \\ 
Model 1 & 0.66^{\ast\ast\ast} & [0.90] &	0.64^{\ast\ast\ast} & [1.94] &	0.65^{\ast\ast\ast} & [3.72] &	0.72^{\ast\ast\ast} & [6.65] \\ 
Model 2 & 0.72^{\ast\ast\ast} & [1.32] &	0.67^{\ast\ast\ast} & [2.98] &	0.67^{\ast\ast\ast} & [5.64] &	0.76^{\ast\ast\ast} & [9.18] \\ 
Model 3 & 0.61^{\ast\ast\ast} & [0.80] &	0.66^{\ast\ast\ast} & [1.76] &	0.60^{\ast\ast\ast} & [3.46] &	0.71^{\ast\ast\ast} & [6.40] \\ 
Model 4 & 0.56^{\ast\ast\ast} & [1.14] &	0.54^{\ast\ast\ast} & [2.57] &	0.56^{\ast\ast\ast} & [4.95] &	0.61^{\ast\ast\ast} & [8.36] \\ 
\hline
\multicolumn{9}{c}{Credit Spread} \\ 
\hline
TVP-VAR-SV & 0.72^{\ast\ast\ast} & [0.59] &	0.72^{\ast\ast\ast} & [1.00] &	0.77^{\ast\ast\ast} & [1.59] &	0.92^{\ast\ast} & [2.69] \\ 
Model 1 & 0.73^{\ast\ast\ast} & [0.56] &	0.72^{\ast\ast\ast} & [0.92] &	0.76^{\ast\ast\ast} & [1.39] &	0.89^{\ast} & [2.15] \\ 
Model 2 & 0.71^{\ast\ast\ast} & [0.78] &	0.78^{\ast\ast\ast} & [1.32] &	0.73^{\ast\ast\ast} & [1.92] &	0.89^{\ast} & [2.75] \\ 
Model 3 & 0.67^{\ast\ast\ast} & [0.49] &	0.64^{\ast\ast\ast} & [0.83] &	0.71^{\ast\ast\ast} & [1.29] &	0.80^{\ast\ast\ast} & [2.03] \\ 
Model 4 & 0.53^{\ast\ast\ast} & [0.69] &	0.53^{\ast\ast\ast} & [1.20] &	0.58^{\ast\ast\ast} & [1.75] &	0.64^{\ast\ast\ast} & [2.53] \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: to be added}
\end{flushleft}
\label{fig:InFevalModel1Prior3Lag5FcstNeval98SamplingMode1DifMode1FacMode1}
\end{table}


==> FcstTables/PaperTableRMSFE_Model_1_Prior_3_Lag_1_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[!t]\centering
\caption{$68\%$ Point Forecast RMSE's ($1$ Lag models)).}
\label{fig:RMSFEModel1Prior3Lag1FcstNeval98SamplingMode1DifMode1FacMode1}
\begin{center}
\begin{tabular}{lllllllll}
\hline\hline
{\textbf{Model}} & {\textbf{1Q}}  & {\textbf{2Q}}   & {\textbf{3Q}}  & {\textbf{4Q}}  & {\textbf{5Q}}  & {\textbf{6Q}}  & {\textbf{7Q}}   & {\textbf{8Q}} \\ 
\hline
\multicolumn{9}{c}{{\textbf{Real GDP}}} \\ 
\hline
TVP-VAR-SV & $0.56$ &	$0.60$  & 	$0.64$  & 	$0.67$  & 	$0.68$  & 	$0.67$  & 	$0.66$  & 	$0.67$  \\ 
GF-TVP-VAR-SV & $1.12^{\ast}$  &	$1.13^{\ast}$  & 	$1.12$  & 	$1.12$  & 	$1.12^{\ast}$  & 	$1.16$  & 	$1.18$  & 	$1.16$ \\ 
CF-TVP-VAR-SV & $1.10$  &	$1.10$  & 	$1.08$  & 	$1.07$  & 	$1.07$  & 	$1.12$  & 	$1.14$  & 	$1.13$ \\ 
\hline
\multicolumn{9}{c}{{\textbf{Inflation}}} \\ 
\hline
TVP-VAR-SV & $0.21$ &	$0.22$  & 	$0.24$  & 	$0.25$  & 	$0.27$  & 	$0.27$  & 	$0.30$  & 	$0.30$  \\ 
GF-TVP-VAR-SV & $0.97$  &	$0.98$  & 	$0.99$  & 	$1.00$  & 	$1.01$  & 	$1.03$  & 	$0.98$  & 	$1.02$ \\ 
CF-TVP-VAR-SV & $0.94$  &	$0.93$  & 	$0.94$  & 	$0.91$  & 	$0.91$  & 	$0.91$  & 	$0.87$  & 	$0.89$ \\ 
\hline
\multicolumn{9}{c}{{\textbf{FFR}}} \\ 
\hline
TVP-VAR-SV & $0.48$ &	$0.91$  & 	$1.26$  & 	$1.60$  & 	$1.90$  & 	$2.17$  & 	$2.42$  & 	$2.64$  \\ 
GF-TVP-VAR-SV & $1.00$  &	$0.97$  & 	$0.95$  & 	$0.94$  & 	$0.94$  & 	$0.94^{\ast}$  & 	$0.94^{\ast}$  & 	$0.95^{\ast\ast}$ \\ 
CF-TVP-VAR-SV & $0.97$  &	$0.93$  & 	$0.92$  & 	$0.91$  & 	$0.91^{\ast}$  & 	$0.91^{\ast\ast}$  & 	$0.90^{\ast\ast\ast}$  & 	$0.90^{\ast\ast\ast}$ \\ 
\hline
\multicolumn{9}{c}{{\textbf{Credit Spread}}} \\ 
\hline
TVP-VAR-SV & $0.35$ &	$0.55$  & 	$0.65$  & 	$0.72$  & 	$0.78$  & 	$0.82$  & 	$0.84$  & 	$0.87$  \\ 
GF-TVP-VAR-SV & $1.01$  &	$1.02$  & 	$1.05$  & 	$1.08$  & 	$1.10^{\ast}$  & 	$1.11^{\ast}$  & 	$1.14^{\ast}$  & 	$1.15^{\ast}$ \\ 
CF-TVP-VAR-SV & $1.01$  &	$1.01$  & 	$1.03$  & 	$1.04$  & 	$1.05$  & 	$1.06$  & 	$1.08^{\ast}$  & 	$1.10^{\ast}$ \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: The forecast evaluation sample is 1987:Q1 to 2011:Q1. We show RMSEs for the benchmark TVP-VAR-SV model in the first line of each panel, and RMSE ratios in the subsequent lines to the respective models. In parentheses we show p-values of Diebold-Mariano tests of equal MSE against the one-sided alternative that the model with time-varying volatility is more accurate, obtained using standard normal critical values. We compute the standard errors entering the Diebold-Mariano statistics using Newey-West.}
\end{flushleft}
\end{table}


==> FcstTables/PaperTableRMSFE_Model_1_Prior_3_Lag_3_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[!t]\centering
\caption{$68\%$ Point Forecast RMSE's ($3$ Lag models)).}
\label{fig:RMSFEModel1Prior3Lag3FcstNeval98SamplingMode1DifMode1FacMode1}
\begin{center}
\begin{tabular}{lllllllll}
\hline\hline
{\textbf{Model}} & {\textbf{1Q}}  & {\textbf{2Q}}   & {\textbf{3Q}}  & {\textbf{4Q}}  & {\textbf{5Q}}  & {\textbf{6Q}}  & {\textbf{7Q}}   & {\textbf{8Q}} \\ 
\hline
\multicolumn{9}{c}{{\textbf{Real GDP}}} \\ 
\hline
TVP-VAR-SV & $0.60$ &	$0.68$  & 	$0.75$  & 	$0.76$  & 	$0.73$  & 	$0.70$  & 	$0.73$  & 	$0.73$  \\ 
GF-TVP-VAR-SV & $1.03^{\ast\ast}$  &	$1.03^{\ast}$  & 	$1.02^{\ast}$  & 	$1.01^{\ast}$  & 	$1.02^{\ast}$  & 	$1.01$  & 	$1.01$  & 	$1.01$ \\ 
CF-TVP-VAR-SV & $1.05^{\ast\ast}$  &	$1.03$  & 	$1.01$  & 	$1.00$  & 	$1.00$  & 	$0.99$  & 	$0.99$  & 	$0.98$ \\ 
\hline
\multicolumn{9}{c}{{\textbf{Inflation}}} \\ 
\hline
TVP-VAR-SV & $0.20$ &	$0.22$  & 	$0.22$  & 	$0.23$  & 	$0.24$  & 	$0.25$  & 	$0.27$  & 	$0.27$  \\ 
GF-TVP-VAR-SV & $0.99$  &	$1.00$  & 	$0.99$  & 	$0.99$  & 	$0.99$  & 	$1.00$  & 	$0.99$  & 	$1.01$ \\ 
CF-TVP-VAR-SV & $0.99$  &	$0.99$  & 	$0.98^{\ast}$  & 	$0.98^{\ast}$  & 	$0.99$  & 	$0.98$  & 	$0.98$  & 	$1.00$ \\ 
\hline
\multicolumn{9}{c}{{\textbf{FFR}}} \\ 
\hline
TVP-VAR-SV & $0.38$ &	$0.77$  & 	$1.13$  & 	$1.48$  & 	$1.78$  & 	$2.04$  & 	$2.26$  & 	$2.44$  \\ 
GF-TVP-VAR-SV & $1.01^{\ast\ast}$  &	$1.02^{\ast}$  & 	$1.02^{\ast}$  & 	$1.02$  & 	$1.02$  & 	$1.02$  & 	$1.02$  & 	$1.02$ \\ 
CF-TVP-VAR-SV & $1.01^{\ast}$  &	$1.02^{\ast}$  & 	$1.02^{\ast}$  & 	$1.01$  & 	$1.02$  & 	$1.02$  & 	$1.02$  & 	$1.02$ \\ 
\hline
\multicolumn{9}{c}{{\textbf{Credit Spread}}} \\ 
\hline
TVP-VAR-SV & $0.36$ &	$0.58$  & 	$0.70$  & 	$0.79$  & 	$0.86$  & 	$0.90$  & 	$0.92$  & 	$0.95$  \\ 
GF-TVP-VAR-SV & $1.00$  &	$1.01$  & 	$1.01$  & 	$1.01$  & 	$1.01$  & 	$1.01^{\ast}$  & 	$1.01^{\ast\ast}$  & 	$1.01$ \\ 
CF-TVP-VAR-SV & $1.00$  &	$1.01$  & 	$1.01$  & 	$1.01$  & 	$1.00$  & 	$1.01$  & 	$1.01^{\ast}$  & 	$1.01^{\ast\ast}$ \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: The forecast evaluation sample is 1987:Q1 to 2011:Q1. We show RMSEs for the benchmark TVP-VAR-SV model in the first line of each panel, and RMSE ratios in the subsequent lines to the respective models. In parentheses we show p-values of Diebold-Mariano tests of equal MSE against the one-sided alternative that the model with time-varying volatility is more accurate, obtained using standard normal critical values. We compute the standard errors entering the Diebold-Mariano statistics using Newey-West.}
\end{flushleft}
\end{table}


==> FcstTables/PaperTableRMSFE_Model_1_Prior_3_Lag_4_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[!t]\centering
\caption{$68\%$ Point Forecast RMSE's ($4$ Lag models)).}
\label{fig:RMSFEModel1Prior3Lag4FcstNeval98SamplingMode1DifMode1FacMode1}
\begin{center}
\begin{tabular}{lllllllll}
\hline\hline
{\textbf{Model}} & {\textbf{1Q}}  & {\textbf{2Q}}   & {\textbf{3Q}}  & {\textbf{4Q}}  & {\textbf{5Q}}  & {\textbf{6Q}}  & {\textbf{7Q}}   & {\textbf{8Q}} \\ 
\hline
\multicolumn{9}{c}{{\textbf{Real GDP}}} \\ 
\hline
TVP-VAR-SV & $0.72$ &	$0.75$  & 	$0.77$  & 	$0.75$  & 	$0.76$  & 	$0.72$  & 	$0.72$  & 	$0.69$  \\ 
GF-TVP-VAR-SV & $1.06$  &	$0.98$  & 	$1.00$  & 	$0.97$  & 	$0.98$  & 	$0.98$  & 	$1.00$  & 	$1.00$ \\ 
CF-TVP-VAR-SV & $1.08$  &	$0.98$  & 	$1.00$  & 	$0.96$  & 	$0.96$  & 	$0.96$  & 	$0.98$  & 	$0.98$ \\ 
\hline
\multicolumn{9}{c}{{\textbf{Inflation}}} \\ 
\hline
TVP-VAR-SV & $0.23$ &	$0.23$  & 	$0.23$  & 	$0.24$  & 	$0.26$  & 	$0.27$  & 	$0.28$  & 	$0.30$  \\ 
GF-TVP-VAR-SV & $0.95^{\ast\ast}$  &	$0.95^{\ast\ast}$  & 	$0.94^{\ast}$  & 	$0.92^{\ast\ast}$  & 	$0.92$  & 	$0.91$  & 	$0.92$  & 	$0.92$ \\ 
CF-TVP-VAR-SV & $0.93^{\ast\ast}$  &	$0.93^{\ast\ast}$  & 	$0.93^{\ast\ast}$  & 	$0.91^{\ast\ast}$  & 	$0.90^{\ast}$  & 	$0.89^{\ast}$  & 	$0.90$  & 	$0.89$ \\ 
\hline
\multicolumn{9}{c}{{\textbf{FFR}}} \\ 
\hline
TVP-VAR-SV & $0.41$ &	$0.79$  & 	$1.13$  & 	$1.49$  & 	$1.83$  & 	$2.13$  & 	$2.42$  & 	$2.67$  \\ 
GF-TVP-VAR-SV & $1.01$  &	$1.04$  & 	$1.05$  & 	$1.04$  & 	$1.04$  & 	$1.03$  & 	$1.02$  & 	$1.00$ \\ 
CF-TVP-VAR-SV & $1.01$  &	$1.07$  & 	$1.09$  & 	$1.08$  & 	$1.07$  & 	$1.06$  & 	$1.04$  & 	$1.02$ \\ 
\hline
\multicolumn{9}{c}{{\textbf{Credit Spread}}} \\ 
\hline
TVP-VAR-SV & $0.36$ &	$0.59$  & 	$0.72$  & 	$0.81$  & 	$0.87$  & 	$0.91$  & 	$0.91$  & 	$0.93$  \\ 
GF-TVP-VAR-SV & $1.01$  &	$1.01$  & 	$1.01$  & 	$1.01$  & 	$1.01$  & 	$1.01$  & 	$1.02$  & 	$1.01$ \\ 
CF-TVP-VAR-SV & $1.01$  &	$1.01$  & 	$1.01$  & 	$1.01$  & 	$1.01$  & 	$1.01$  & 	$1.02$  & 	$1.01$ \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: The forecast evaluation sample is 1987:Q1 to 2011:Q1. We show RMSEs for the benchmark TVP-VAR-SV model in the first line of each panel, and RMSE ratios in the subsequent lines to the respective models. In parentheses we show p-values of Diebold-Mariano tests of equal MSE against the one-sided alternative that the model with time-varying volatility is more accurate, obtained using standard normal critical values. We compute the standard errors entering the Diebold-Mariano statistics using Newey-West.}
\end{flushleft}
\end{table}


==> FcstTables/Table2CRPS_Model_1_Prior_3_Lag_1_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[!t]\centering
\caption{Density forecast accuracy as measured by CRPS ($1$ Lag models).}
\label{fig:CRPSModel1Prior3Lag1FcstNeval98SamplingMode1DifMode1FacMode1}
\begin{center}
\begin{tabular}{l *{4}{d{3.3}} }
\hline\hline
\textbf{Model} & \textbf{1Q}  & \textbf{2Q}  & \textbf{4Q}  & \textbf{8Q} \\ 
\hline
\multicolumn{5}{c}{Real GDP} \\ 
\hline
TVP-VAR-SV & 0.31 & 	0.33 & 	0.36 & 	0.38  \\ 
GF-TVP-VAR-SV & -9.77^{\ast\ast} & 	-14.26^{\ast\ast\ast}  & 	-13.65^{\ast\ast}  & 	-13.67  \\ 
CF-TVP-VAR-SV & -6.14 & 	-9.15^{\ast\ast}  & 	-7.78^{\ast}  & 	-9.51  \\ 
\hline
\multicolumn{5}{c}{Inflation} \\ 
\hline
TVP-VAR-SV & 0.12 & 	0.13 & 	0.15 & 	0.18  \\ 
GF-TVP-VAR-SV & -0.42 & 	-2.08  & 	-2.24  & 	-1.39  \\ 
CF-TVP-VAR-SV & 3.60 & 	2.12  & 	5.38  & 	8.08  \\ 
\hline
\multicolumn{5}{c}{FFR} \\ 
\hline
TVP-VAR-SV & 0.24 & 	0.47 & 	0.86 & 	1.44  \\ 
GF-TVP-VAR-SV & -1.20 & 	2.28  & 	4.26^{\ast}  & 	4.71^{\ast}  \\ 
CF-TVP-VAR-SV & -2.51 & 	2.32  & 	5.86^{\ast\ast}  & 	8.36^{\ast\ast\ast}  \\ 
\hline
\multicolumn{5}{c}{Credit Spread} \\ 
\hline
TVP-VAR-SV & 0.16 & 	0.26 & 	0.36 & 	0.45  \\ 
GF-TVP-VAR-SV & -0.42 & 	-2.74  & 	-8.51^{\ast}  & 	-17.10^{\ast\ast}  \\ 
CF-TVP-VAR-SV & -0.34 & 	-1.71  & 	-5.08  & 	-9.14^{\ast\ast}  \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: The table reports CRPS results for out-of-sample density forecasts. The sample uses predictions made from the date X through X. For each variable, the rows for Model 1-Model 4 reports the relative CRPS calculated as the percentage decrease of the CRPS when using the respective model rather than the benchmark TVP-VAR; positive numbers indicate improvement over the benchmark TVP-VAR case. The respective first rows reports the CRPS for the benchmark TVP-VAR case. Statistical significance of the differences in average CRPS assessed with a Diebold and Mariano (1995) test is indicated by the corresponding numbers in brakets.}
\end{flushleft}
\end{table}


==> FcstTables/Table2CRPS_Model_1_Prior_3_Lag_3_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[!t]\centering
\caption{Density forecast accuracy as measured by CRPS ($3$ Lag models).}
\label{fig:CRPSModel1Prior3Lag3FcstNeval98SamplingMode1DifMode1FacMode1}
\begin{center}
\begin{tabular}{l *{4}{d{3.3}} }
\hline\hline
\textbf{Model} & \textbf{1Q}  & \textbf{2Q}  & \textbf{4Q}  & \textbf{8Q} \\ 
\hline
\multicolumn{5}{c}{Real GDP} \\ 
\hline
TVP-VAR-SV & 0.33 & 	0.36 & 	0.40 & 	0.39  \\ 
GF-TVP-VAR-SV & -2.33^{\ast} & 	-2.27^{\ast\ast}  & 	-1.52  & 	-0.13  \\ 
CF-TVP-VAR-SV & -3.13^{\ast\ast} & 	-2.70^{\ast}  & 	-1.61  & 	1.33  \\ 
\hline
\multicolumn{5}{c}{Inflation} \\ 
\hline
TVP-VAR-SV & 0.11 & 	0.12 & 	0.13 & 	0.17  \\ 
GF-TVP-VAR-SV & 0.63 & 	-0.25  & 	0.83  & 	-0.94  \\ 
CF-TVP-VAR-SV & -0.25 & 	-1.04  & 	0.78  & 	-0.15  \\ 
\hline
\multicolumn{5}{c}{FFR} \\ 
\hline
TVP-VAR-SV & 0.20 & 	0.43 & 	0.84 & 	1.41  \\ 
GF-TVP-VAR-SV & -0.85^{\ast\ast} & 	-1.62^{\ast\ast}  & 	-1.53  & 	-1.96  \\ 
CF-TVP-VAR-SV & -2.57 & 	-1.62  & 	-1.13  & 	-1.61  \\ 
\hline
\multicolumn{5}{c}{Credit Spread} \\ 
\hline
TVP-VAR-SV & 0.16 & 	0.28 & 	0.39 & 	0.48  \\ 
GF-TVP-VAR-SV & 0.18 & 	0.04  & 	-1.32  & 	-1.68  \\ 
CF-TVP-VAR-SV & -0.88 & 	-1.78  & 	-2.71^{\ast\ast}  & 	-1.32  \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: The table reports CRPS results for out-of-sample density forecasts. The sample uses predictions made from the date X through X. For each variable, the rows for Model 1-Model 4 reports the relative CRPS calculated as the percentage decrease of the CRPS when using the respective model rather than the benchmark TVP-VAR; positive numbers indicate improvement over the benchmark TVP-VAR case. The respective first rows reports the CRPS for the benchmark TVP-VAR case. Statistical significance of the differences in average CRPS assessed with a Diebold and Mariano (1995) test is indicated by the corresponding numbers in brakets.}
\end{flushleft}
\end{table}


==> FcstTables/Table2CRPS_Model_1_Prior_3_Lag_4_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[!t]\centering
\caption{Density forecast accuracy as measured by CRPS ($4$ Lag models).}
\label{fig:CRPSModel1Prior3Lag4FcstNeval98SamplingMode1DifMode1FacMode1}
\begin{center}
\begin{tabular}{l *{4}{d{3.3}} }
\hline\hline
\textbf{Model} & \textbf{1Q}  & \textbf{2Q}  & \textbf{4Q}  & \textbf{8Q} \\ 
\hline
\multicolumn{5}{c}{Real GDP} \\ 
\hline
TVP-VAR-SV & 0.37 & 	0.39 & 	0.41 & 	0.43  \\ 
GF-TVP-VAR-SV & -8.89^{\ast} & 	-1.99  & 	1.93  & 	4.37  \\ 
CF-TVP-VAR-SV & -13.21^{\ast\ast} & 	-1.55  & 	3.67  & 	7.90  \\ 
\hline
\multicolumn{5}{c}{Inflation} \\ 
\hline
TVP-VAR-SV & 0.12 & 	0.13 & 	0.14 & 	0.18  \\ 
GF-TVP-VAR-SV & 3.98^{\ast} & 	4.91^{\ast}  & 	6.57^{\ast\ast}  & 	6.47  \\ 
CF-TVP-VAR-SV & 5.00^{\ast} & 	6.57^{\ast\ast}  & 	8.23^{\ast\ast}  & 	9.86^{\ast\ast}  \\ 
\hline
\multicolumn{5}{c}{FFR} \\ 
\hline
TVP-VAR-SV & 0.21 & 	0.43 & 	0.83 & 	1.49  \\ 
GF-TVP-VAR-SV & -3.19 & 	-5.47  & 	-6.27  & 	-1.80  \\ 
CF-TVP-VAR-SV & -8.81^{\ast} & 	-10.73  & 	-11.07  & 	-4.62  \\ 
\hline
\multicolumn{5}{c}{Credit Spread} \\ 
\hline
TVP-VAR-SV & 0.17 & 	0.28 & 	0.40 & 	0.47  \\ 
GF-TVP-VAR-SV & -0.86 & 	-1.14  & 	-2.95  & 	-2.73  \\ 
CF-TVP-VAR-SV & -2.16 & 	-3.56  & 	-5.37  & 	-2.94  \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: The table reports CRPS results for out-of-sample density forecasts. The sample uses predictions made from the date X through X. For each variable, the rows for Model 1-Model 4 reports the relative CRPS calculated as the percentage decrease of the CRPS when using the respective model rather than the benchmark TVP-VAR; positive numbers indicate improvement over the benchmark TVP-VAR case. The respective first rows reports the CRPS for the benchmark TVP-VAR case. Statistical significance of the differences in average CRPS assessed with a Diebold and Mariano (1995) test is indicated by the corresponding numbers in brakets.}
\end{flushleft}
\end{table}


==> FcstTables/Table2InFevalCTestHorizon_1_Model_1_Prior_3_Lag_1_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[!t]\centering
\caption{$68\%$ Christoffersen Likelihood-Ratio Tests ($1$ Lags, horizon $1$)).}
\label{tab:InFevalCTestHorizon1Model1Prior3Lag1FcstNeval98SamplingMode1DifMode1FacMode1}
\begin{center}
\begin{tabular}{l *{3}{d{6.6}} }
\hline\hline
\multicolumn{1}{l}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Coverage}}  & \multicolumn{1}{c}{\textbf{Independence}}  & \multicolumn{1}{c}{\textbf{Joint}} \\ 
\hline
\multicolumn{4}{c}{\textbf{Real GDP}} \\ 
\hline
TVP-VAR-SV & 15.08^{\ast\ast\ast} &  0.26 &  15.34^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 18.88^{\ast\ast\ast} &  0.01 &  18.89^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 13.32^{\ast\ast\ast} &  0.66 &  13.98^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Inflation}} \\ 
\hline
TVP-VAR-SV & 4.88^{\ast\ast} &  0.19 &  5.07^{\ast} \\ 
GF-TVP-VAR-SV & 6.03^{\ast\ast} &  0.61 &  6.63^{\ast\ast} \\ 
CF-TVP-VAR-SV & 1.44 &  0.51 &  1.95 \\ 
\hline
\multicolumn{4}{c}{\textbf{FFR}} \\ 
\hline
TVP-VAR-SV & 16.93^{\ast\ast\ast} &  6.11^{\ast\ast} &  23.04^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 18.88^{\ast\ast\ast} &  0.01 &  18.89^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 8.64^{\ast\ast\ast} &  0.55 &  9.19^{\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Credit Spread}} \\ 
\hline
TVP-VAR-SV & 15.08^{\ast\ast\ast} &  0.01 &  15.09^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 20.92^{\ast\ast\ast} &  0.01 &  20.93^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 25.26^{\ast\ast\ast} &  0.51 &  25.77^{\ast\ast\ast} \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: to be added}
\end{flushleft}
\end{table}


==> FcstTables/Table2InFevalCTestHorizon_1_Model_1_Prior_3_Lag_3_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[!t]\centering
\caption{$68\%$ Christoffersen Likelihood-Ratio Tests ($3$ Lags, horizon $1$)).}
\label{tab:InFevalCTestHorizon1Model1Prior3Lag3FcstNeval98SamplingMode1DifMode1FacMode1}
\begin{center}
\begin{tabular}{l *{3}{d{6.6}} }
\hline\hline
\multicolumn{1}{l}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Coverage}}  & \multicolumn{1}{c}{\textbf{Independence}}  & \multicolumn{1}{c}{\textbf{Joint}} \\ 
\hline
\multicolumn{4}{c}{\textbf{Real GDP}} \\ 
\hline
TVP-VAR-SV & 11.66^{\ast\ast\ast} &  1.75 &  13.41^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 13.32^{\ast\ast\ast} &  3.01^{\ast} &  16.33^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 13.32^{\ast\ast\ast} &  1.54 &  14.86^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Inflation}} \\ 
\hline
TVP-VAR-SV & 1.44 &  0.98 &  2.41 \\ 
GF-TVP-VAR-SV & 1.44 &  1.27 &  2.70 \\ 
CF-TVP-VAR-SV & 2.92^{\ast} &  4.93^{\ast\ast} &  7.85^{\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{FFR}} \\ 
\hline
TVP-VAR-SV & 15.08^{\ast\ast\ast} &  0.04 &  15.12^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 11.66^{\ast\ast\ast} &  0.09 &  11.76^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 4.88^{\ast\ast} &  0.51 &  5.39^{\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Credit Spread}} \\ 
\hline
TVP-VAR-SV & 15.08^{\ast\ast\ast} &  0.01 &  15.09^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 15.08^{\ast\ast\ast} &  0.18 &  15.26^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 20.92^{\ast\ast\ast} &  2.34 &  23.26^{\ast\ast\ast} \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: to be added}
\end{flushleft}
\end{table}


==> FcstTables/Table2InFevalCTestHorizon_1_Model_1_Prior_3_Lag_4_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[!t]\centering
\caption{$68\%$ Christoffersen Likelihood-Ratio Tests ($4$ Lags, horizon $1$)).}
\label{tab:InFevalCTestHorizon1Model1Prior3Lag4FcstNeval98SamplingMode1DifMode1FacMode1}
\begin{center}
\begin{tabular}{l *{3}{d{6.6}} }
\hline\hline
\multicolumn{1}{l}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Coverage}}  & \multicolumn{1}{c}{\textbf{Independence}}  & \multicolumn{1}{c}{\textbf{Joint}} \\ 
\hline
\multicolumn{4}{c}{\textbf{Real GDP}} \\ 
\hline
TVP-VAR-SV & 8.64^{\ast\ast\ast} &  0.06 &  8.70^{\ast\ast} \\ 
GF-TVP-VAR-SV & 29.96^{\ast\ast\ast} &  1.33 &  31.29^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 40.39^{\ast\ast\ast} &  0.32 &  40.72^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Inflation}} \\ 
\hline
TVP-VAR-SV & 3.84^{\ast\ast} &  0.51 &  4.35 \\ 
GF-TVP-VAR-SV & 2.12 &  0.11 &  2.23 \\ 
CF-TVP-VAR-SV & 1.44 &  0.29 &  1.72 \\ 
\hline
\multicolumn{4}{c}{\textbf{FFR}} \\ 
\hline
TVP-VAR-SV & 4.88^{\ast\ast} &  0.15 &  5.03^{\ast} \\ 
GF-TVP-VAR-SV & 13.32^{\ast\ast\ast} &  0.93 &  14.26^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 7.28^{\ast\ast\ast} &  4.79^{\ast\ast} &  12.07^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Credit Spread}} \\ 
\hline
TVP-VAR-SV & 10.10^{\ast\ast\ast} &  0.00 &  10.10^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 15.08^{\ast\ast\ast} &  0.57 &  15.65^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 15.08^{\ast\ast\ast} &  0.44 &  15.52^{\ast\ast\ast} \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: to be added}
\end{flushleft}
\end{table}


==> FcstTables/Table2InFevalCTestHorizon_1_Model_2_Prior_3_Lag_1_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[!t]\centering
\caption{$68\%$ Christoffersen Likelihood-Ratio Tests ($1$ Lags, horizon $2$)).}
\label{tab:InFevalCTestHorizon2Model1Prior3Lag1FcstNeval98SamplingMode1DifMode1FacMode1}
\begin{center}
\begin{tabular}{l *{3}{d{6.6}} }
\hline\hline
\multicolumn{1}{l}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Coverage}}  & \multicolumn{1}{c}{\textbf{Independence}}  & \multicolumn{1}{c}{\textbf{Joint}} \\ 
\hline
\multicolumn{4}{c}{\textbf{Real GDP}} \\ 
\hline
TVP-VAR-SV & 15.08^{\ast\ast\ast} &  0.94 &  16.02^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 20.92^{\ast\ast\ast} &  0.41 &  21.33^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 15.08^{\ast\ast\ast} &  2.52 &  17.60^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Inflation}} \\ 
\hline
TVP-VAR-SV & 2.92^{\ast} &  2.82^{\ast} &  5.74^{\ast} \\ 
GF-TVP-VAR-SV & 6.03^{\ast\ast} &  2.18 &  8.20^{\ast\ast} \\ 
CF-TVP-VAR-SV & 3.84^{\ast\ast} &  12.21^{\ast\ast\ast} &  16.05^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{FFR}} \\ 
\hline
TVP-VAR-SV & 23.05^{\ast\ast\ast} &  12.23^{\ast\ast\ast} &  35.28^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 18.88^{\ast\ast\ast} &  5.86^{\ast\ast} &  24.74^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 20.92^{\ast\ast\ast} &  7.25^{\ast\ast\ast} &  28.17^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Credit Spread}} \\ 
\hline
TVP-VAR-SV & 27.57^{\ast\ast\ast} &  4.40^{\ast\ast} &  31.96^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 25.26^{\ast\ast\ast} &  5.97^{\ast\ast} &  31.23^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 27.57^{\ast\ast\ast} &  8.76^{\ast\ast\ast} &  36.33^{\ast\ast\ast} \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: to be added}
\end{flushleft}
\end{table}


==> FcstTables/Table2InFevalCTestHorizon_1_Model_2_Prior_3_Lag_2_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[!t]\centering
\caption{$68\%$ Christoffersen Likelihood-Ratio Tests ($2$ Lags, horizon $2$)).}
\label{tab:InFevalCTestHorizon2Model1Prior3Lag2FcstNeval98SamplingMode1DifMode1FacMode1}
\begin{center}
\begin{tabular}{l *{3}{d{6.6}} }
\hline\hline
\multicolumn{1}{l}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Coverage}}  & \multicolumn{1}{c}{\textbf{Independence}}  & \multicolumn{1}{c}{\textbf{Joint}} \\ 
\hline
\multicolumn{4}{c}{\textbf{Real GDP}} \\ 
\hline
TVP-VAR-SV & 18.88^{\ast\ast\ast} &  1.55 &  20.43^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 18.88^{\ast\ast\ast} &  2.86^{\ast} &  21.74^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 16.93^{\ast\ast\ast} &  1.24 &  18.17^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Inflation}} \\ 
\hline
TVP-VAR-SV & 10.10^{\ast\ast\ast} &  5.66^{\ast\ast} &  15.76^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 13.32^{\ast\ast\ast} &  3.62^{\ast} &  16.95^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 4.88^{\ast\ast} &  10.03^{\ast\ast\ast} &  14.91^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{FFR}} \\ 
\hline
TVP-VAR-SV & 11.66^{\ast\ast\ast} &  12.09^{\ast\ast\ast} &  23.75^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 10.10^{\ast\ast\ast} &  11.13^{\ast\ast\ast} &  21.23^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 4.88^{\ast\ast} &  10.03^{\ast\ast\ast} &  14.91^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Credit Spread}} \\ 
\hline
TVP-VAR-SV & 29.96^{\ast\ast\ast} &  3.06^{\ast} &  33.02^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 29.96^{\ast\ast\ast} &  5.53^{\ast\ast} &  35.50^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 27.57^{\ast\ast\ast} &  9.86^{\ast\ast\ast} &  37.43^{\ast\ast\ast} \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: to be added}
\end{flushleft}
\end{table}


==> FcstTables/Table2InFevalCTestHorizon_1_Model_2_Prior_3_Lag_3_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[!t]\centering
\caption{$68\%$ Christoffersen Likelihood-Ratio Tests ($3$ Lags, horizon $2$)).}
\label{tab:InFevalCTestHorizon2Model1Prior3Lag3FcstNeval98SamplingMode1DifMode1FacMode1}
\begin{center}
\begin{tabular}{l *{3}{d{6.6}} }
\hline\hline
\multicolumn{1}{l}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Coverage}}  & \multicolumn{1}{c}{\textbf{Independence}}  & \multicolumn{1}{c}{\textbf{Joint}} \\ 
\hline
\multicolumn{4}{c}{\textbf{Real GDP}} \\ 
\hline
TVP-VAR-SV & 8.64^{\ast\ast\ast} &  2.97^{\ast} &  11.61^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 10.10^{\ast\ast\ast} &  3.61^{\ast} &  13.71^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 10.10^{\ast\ast\ast} &  5.66^{\ast\ast} &  15.76^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Inflation}} \\ 
\hline
TVP-VAR-SV & 7.28^{\ast\ast\ast} &  9.13^{\ast\ast\ast} &  16.41^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 7.28^{\ast\ast\ast} &  9.13^{\ast\ast\ast} &  16.41^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 7.28^{\ast\ast\ast} &  16.12^{\ast\ast\ast} &  23.40^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{FFR}} \\ 
\hline
TVP-VAR-SV & 10.10^{\ast\ast\ast} &  3.61^{\ast} &  13.71^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 10.10^{\ast\ast\ast} &  3.61^{\ast} &  13.71^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 7.28^{\ast\ast\ast} &  2.35 &  9.63^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Credit Spread}} \\ 
\hline
TVP-VAR-SV & 18.88^{\ast\ast\ast} &  6.69^{\ast\ast\ast} &  25.57^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 20.92^{\ast\ast\ast} &  7.25^{\ast\ast\ast} &  28.17^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 23.05^{\ast\ast\ast} &  20.93^{\ast\ast\ast} &  43.97^{\ast\ast\ast} \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: to be added}
\end{flushleft}
\end{table}


==> FcstTables/Table2InFevalCTestHorizon_1_Model_2_Prior_3_Lag_4_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[!t]\centering
\caption{$68\%$ Christoffersen Likelihood-Ratio Tests ($4$ Lags, horizon $2$)).}
\label{tab:InFevalCTestHorizon2Model1Prior3Lag4FcstNeval98SamplingMode1DifMode1FacMode1}
\begin{center}
\begin{tabular}{l *{3}{d{6.6}} }
\hline\hline
\multicolumn{1}{l}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Coverage}}  & \multicolumn{1}{c}{\textbf{Independence}}  & \multicolumn{1}{c}{\textbf{Joint}} \\ 
\hline
\multicolumn{4}{c}{\textbf{Real GDP}} \\ 
\hline
TVP-VAR-SV & 7.28^{\ast\ast\ast} &  1.07 &  8.35^{\ast\ast} \\ 
GF-TVP-VAR-SV & 11.66^{\ast\ast\ast} &  4.25^{\ast\ast} &  15.91^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 18.88^{\ast\ast\ast} &  5.32^{\ast\ast} &  24.20^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Inflation}} \\ 
\hline
TVP-VAR-SV & 2.92^{\ast} &  2.82^{\ast} &  5.74^{\ast} \\ 
GF-TVP-VAR-SV & 2.12 &  0.07 &  2.19 \\ 
CF-TVP-VAR-SV & 2.12 &  0.72 &  2.84 \\ 
\hline
\multicolumn{4}{c}{\textbf{FFR}} \\ 
\hline
TVP-VAR-SV & 10.10^{\ast\ast\ast} &  3.61^{\ast} &  13.71^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 18.88^{\ast\ast\ast} &  5.32^{\ast\ast} &  24.20^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 13.32^{\ast\ast\ast} &  27.28^{\ast\ast\ast} &  40.60^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Credit Spread}} \\ 
\hline
TVP-VAR-SV & 16.93^{\ast\ast\ast} &  8.55^{\ast\ast\ast} &  25.49^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 25.26^{\ast\ast\ast} &  4.76^{\ast\ast} &  30.02^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 27.57^{\ast\ast\ast} &  12.80^{\ast\ast\ast} &  40.37^{\ast\ast\ast} \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: to be added}
\end{flushleft}
\end{table}


==> FcstTables/Table2InFevalCTestHorizon_1_Model_2_Prior_3_Lag_5_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[!t]\centering
\caption{$68\%$ Christoffersen Likelihood-Ratio Tests ($5$ Lags, horizon $2$)).}
\label{tab:InFevalCTestHorizon2Model1Prior3Lag5FcstNeval98SamplingMode1DifMode1FacMode1}
\begin{center}
\begin{tabular}{l *{3}{d{6.6}} }
\hline\hline
\multicolumn{1}{l}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Coverage}}  & \multicolumn{1}{c}{\textbf{Independence}}  & \multicolumn{1}{c}{\textbf{Joint}} \\ 
\hline
\multicolumn{4}{c}{\textbf{Real GDP}} \\ 
\hline
TVP-VAR-SV & 0.51 &  0.05 &  0.56 \\ 
GF-TVP-VAR-SV & 0.16 &  6.72^{\ast\ast\ast} &  6.89^{\ast\ast} \\ 
CF-TVP-VAR-SV & 1.44 &  8.04^{\ast\ast\ast} &  9.47^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Inflation}} \\ 
\hline
TVP-VAR-SV & 0.16 &  0.00 &  0.16 \\ 
GF-TVP-VAR-SV & 3.74^{\ast} &  0.04 &  3.78 \\ 
CF-TVP-VAR-SV & 0.18 &  2.25 &  2.43 \\ 
\hline
\multicolumn{4}{c}{\textbf{FFR}} \\ 
\hline
TVP-VAR-SV & 1.44 &  5.16^{\ast\ast} &  6.60^{\ast\ast} \\ 
GF-TVP-VAR-SV & 23.05^{\ast\ast\ast} &  18.56^{\ast\ast\ast} &  41.61^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 18.88^{\ast\ast\ast} &  25.53^{\ast\ast\ast} &  44.41^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Credit Spread}} \\ 
\hline
TVP-VAR-SV & 7.28^{\ast\ast\ast} &  1.07 &  8.35^{\ast\ast} \\ 
GF-TVP-VAR-SV & 8.64^{\ast\ast\ast} &  5.62^{\ast\ast} &  14.26^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 20.92^{\ast\ast\ast} &  20.17^{\ast\ast\ast} &  41.08^{\ast\ast\ast} \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: to be added}
\end{flushleft}
\end{table}


==> FcstTables/Table2InFevalCTestHorizon_1_Model_4_Prior_3_Lag_1_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[!t]\centering
\caption{$68\%$ Christoffersen Likelihood-Ratio Tests ($1$ Lags, horizon $4$)).}
\label{tab:InFevalCTestHorizon4Model1Prior3Lag1FcstNeval98SamplingMode1DifMode1FacMode1}
\begin{center}
\begin{tabular}{l *{3}{d{6.6}} }
\hline\hline
\multicolumn{1}{l}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Coverage}}  & \multicolumn{1}{c}{\textbf{Independence}}  & \multicolumn{1}{c}{\textbf{Joint}} \\ 
\hline
\multicolumn{4}{c}{\textbf{Real GDP}} \\ 
\hline
TVP-VAR-SV & 3.84^{\ast\ast} &  3.68^{\ast} &  7.53^{\ast\ast} \\ 
GF-TVP-VAR-SV & 25.26^{\ast\ast\ast} &  1.72 &  26.98^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 15.08^{\ast\ast\ast} &  2.04 &  17.12^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Inflation}} \\ 
\hline
TVP-VAR-SV & 1.44 &  1.27 &  2.70 \\ 
GF-TVP-VAR-SV & 1.44 &  5.16^{\ast\ast} &  6.60^{\ast\ast} \\ 
CF-TVP-VAR-SV & 0.88 &  9.93^{\ast\ast\ast} &  10.81^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{FFR}} \\ 
\hline
TVP-VAR-SV & 27.57^{\ast\ast\ast} &  20.54^{\ast\ast\ast} &  48.11^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 29.96^{\ast\ast\ast} &  21.10^{\ast\ast\ast} &  51.06^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 18.88^{\ast\ast\ast} &  23.65^{\ast\ast\ast} &  42.53^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Credit Spread}} \\ 
\hline
TVP-VAR-SV & 11.66^{\ast\ast\ast} &  21.30^{\ast\ast\ast} &  32.96^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 16.93^{\ast\ast\ast} &  29.52^{\ast\ast\ast} &  46.46^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 29.96^{\ast\ast\ast} &  34.77^{\ast\ast\ast} &  64.73^{\ast\ast\ast} \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: to be added}
\end{flushleft}
\end{table}


==> FcstTables/Table2InFevalCTestHorizon_1_Model_4_Prior_3_Lag_2_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[!t]\centering
\caption{$68\%$ Christoffersen Likelihood-Ratio Tests ($2$ Lags, horizon $4$)).}
\label{tab:InFevalCTestHorizon4Model1Prior3Lag2FcstNeval98SamplingMode1DifMode1FacMode1}
\begin{center}
\begin{tabular}{l *{3}{d{6.6}} }
\hline\hline
\multicolumn{1}{l}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Coverage}}  & \multicolumn{1}{c}{\textbf{Independence}}  & \multicolumn{1}{c}{\textbf{Joint}} \\ 
\hline
\multicolumn{4}{c}{\textbf{Real GDP}} \\ 
\hline
TVP-VAR-SV & 2.12 &  0.72 &  2.84 \\ 
GF-TVP-VAR-SV & 8.64^{\ast\ast\ast} &  2.97^{\ast} &  11.61^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 11.66^{\ast\ast\ast} &  0.41 &  12.07^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Inflation}} \\ 
\hline
TVP-VAR-SV & 0.45 &  0.19 &  0.64 \\ 
GF-TVP-VAR-SV & 2.12 &  2.01 &  4.12 \\ 
CF-TVP-VAR-SV & 0.16 &  1.81 &  1.97 \\ 
\hline
\multicolumn{4}{c}{\textbf{FFR}} \\ 
\hline
TVP-VAR-SV & 13.32^{\ast\ast\ast} &  25.33^{\ast\ast\ast} &  38.66^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 16.93^{\ast\ast\ast} &  27.45^{\ast\ast\ast} &  44.39^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 16.93^{\ast\ast\ast} &  18.49^{\ast\ast\ast} &  35.43^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Credit Spread}} \\ 
\hline
TVP-VAR-SV & 18.88^{\ast\ast\ast} &  36.12^{\ast\ast\ast} &  55.00^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 20.92^{\ast\ast\ast} &  43.33^{\ast\ast\ast} &  64.25^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 32.44^{\ast\ast\ast} &  54.60^{\ast\ast\ast} &  87.04^{\ast\ast\ast} \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: to be added}
\end{flushleft}
\end{table}


==> FcstTables/Table2InFevalCTestHorizon_1_Model_4_Prior_3_Lag_3_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[!t]\centering
\caption{$68\%$ Christoffersen Likelihood-Ratio Tests ($3$ Lags, horizon $4$)).}
\label{tab:InFevalCTestHorizon4Model1Prior3Lag3FcstNeval98SamplingMode1DifMode1FacMode1}
\begin{center}
\begin{tabular}{l *{3}{d{6.6}} }
\hline\hline
\multicolumn{1}{l}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Coverage}}  & \multicolumn{1}{c}{\textbf{Independence}}  & \multicolumn{1}{c}{\textbf{Joint}} \\ 
\hline
\multicolumn{4}{c}{\textbf{Real GDP}} \\ 
\hline
TVP-VAR-SV & 6.03^{\ast\ast} &  3.37^{\ast} &  9.39^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 7.28^{\ast\ast\ast} &  2.35 &  9.63^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 8.64^{\ast\ast\ast} &  1.53 &  10.17^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Inflation}} \\ 
\hline
TVP-VAR-SV & 0.16 &  0.48 &  0.65 \\ 
GF-TVP-VAR-SV & 0.16 &  0.48 &  0.65 \\ 
CF-TVP-VAR-SV & 0.16 &  1.81 &  1.97 \\ 
\hline
\multicolumn{4}{c}{\textbf{FFR}} \\ 
\hline
TVP-VAR-SV & 20.92^{\ast\ast\ast} &  9.85^{\ast\ast\ast} &  30.76^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 25.26^{\ast\ast\ast} &  17.66^{\ast\ast\ast} &  42.92^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 18.88^{\ast\ast\ast} &  19.36^{\ast\ast\ast} &  38.24^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Credit Spread}} \\ 
\hline
TVP-VAR-SV & 20.92^{\ast\ast\ast} &  37.13^{\ast\ast\ast} &  58.05^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 25.26^{\ast\ast\ast} &  38.96^{\ast\ast\ast} &  64.23^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 29.96^{\ast\ast\ast} &  40.53^{\ast\ast\ast} &  70.49^{\ast\ast\ast} \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: to be added}
\end{flushleft}
\end{table}


==> FcstTables/Table2InFevalCTestHorizon_1_Model_4_Prior_3_Lag_4_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[!t]\centering
\caption{$68\%$ Christoffersen Likelihood-Ratio Tests ($4$ Lags, horizon $4$)).}
\label{tab:InFevalCTestHorizon4Model1Prior3Lag4FcstNeval98SamplingMode1DifMode1FacMode1}
\begin{center}
\begin{tabular}{l *{3}{d{6.6}} }
\hline\hline
\multicolumn{1}{l}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Coverage}}  & \multicolumn{1}{c}{\textbf{Independence}}  & \multicolumn{1}{c}{\textbf{Joint}} \\ 
\hline
\multicolumn{4}{c}{\textbf{Real GDP}} \\ 
\hline
TVP-VAR-SV & 0.88 &  3.98^{\ast\ast} &  4.85^{\ast} \\ 
GF-TVP-VAR-SV & 1.44 &  2.90^{\ast} &  4.34 \\ 
CF-TVP-VAR-SV & 2.92^{\ast} &  2.82^{\ast} &  5.74^{\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Inflation}} \\ 
\hline
TVP-VAR-SV & 0.18 &  0.59 &  0.77 \\ 
GF-TVP-VAR-SV & 0.18 &  0.59 &  0.77 \\ 
CF-TVP-VAR-SV & 0.02 &  0.26 &  0.28 \\ 
\hline
\multicolumn{4}{c}{\textbf{FFR}} \\ 
\hline
TVP-VAR-SV & 4.88^{\ast\ast} &  17.62^{\ast\ast\ast} &  22.50^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 20.92^{\ast\ast\ast} &  14.17^{\ast\ast\ast} &  35.09^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 27.57^{\ast\ast\ast} &  19.93^{\ast\ast\ast} &  47.50^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Credit Spread}} \\ 
\hline
TVP-VAR-SV & 10.10^{\ast\ast\ast} &  30.06^{\ast\ast\ast} &  40.16^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 16.93^{\ast\ast\ast} &  35.04^{\ast\ast\ast} &  51.97^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 25.26^{\ast\ast\ast} &  45.24^{\ast\ast\ast} &  70.51^{\ast\ast\ast} \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: to be added}
\end{flushleft}
\end{table}


==> FcstTables/Table2InFevalCTestHorizon_1_Model_4_Prior_3_Lag_5_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[!t]\centering
\caption{$68\%$ Christoffersen Likelihood-Ratio Tests ($5$ Lags, horizon $4$)).}
\label{tab:InFevalCTestHorizon4Model1Prior3Lag5FcstNeval98SamplingMode1DifMode1FacMode1}
\begin{center}
\begin{tabular}{l *{3}{d{6.6}} }
\hline\hline
\multicolumn{1}{l}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Coverage}}  & \multicolumn{1}{c}{\textbf{Independence}}  & \multicolumn{1}{c}{\textbf{Joint}} \\ 
\hline
\multicolumn{4}{c}{\textbf{Real GDP}} \\ 
\hline
TVP-VAR-SV & 11.02^{\ast\ast\ast} &  6.22^{\ast\ast} &  17.24^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 6.75^{\ast\ast\ast} &  3.29^{\ast} &  10.04^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 5.11^{\ast\ast} &  2.30 &  7.41^{\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Inflation}} \\ 
\hline
TVP-VAR-SV & 6.75^{\ast\ast\ast} &  3.29^{\ast} &  10.04^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 3.74^{\ast} &  0.04 &  3.78 \\ 
CF-TVP-VAR-SV & 2.61 &  0.94 &  3.56 \\ 
\hline
\multicolumn{4}{c}{\textbf{FFR}} \\ 
\hline
TVP-VAR-SV & 0.45 &  12.08^{\ast\ast\ast} &  12.53^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 20.92^{\ast\ast\ast} &  31.52^{\ast\ast\ast} &  52.44^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 32.44^{\ast\ast\ast} &  47.59^{\ast\ast\ast} &  80.03^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Credit Spread}} \\ 
\hline
TVP-VAR-SV & 3.84^{\ast\ast} &  17.59^{\ast\ast\ast} &  21.43^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 4.88^{\ast\ast} &  42.81^{\ast\ast\ast} &  47.69^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 10.10^{\ast\ast\ast} &  30.06^{\ast\ast\ast} &  40.16^{\ast\ast\ast} \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: to be added}
\end{flushleft}
\end{table}


==> FcstTables/Table2InFevalCTestHorizon_1_Model_8_Prior_3_Lag_1_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[!t]\centering
\caption{$68\%$ Christoffersen Likelihood-Ratio Tests ($1$ Lags, horizon $8$)).}
\label{tab:InFevalCTestHorizon8Model1Prior3Lag1FcstNeval98SamplingMode1DifMode1FacMode1}
\begin{center}
\begin{tabular}{l *{3}{d{6.6}} }
\hline\hline
\multicolumn{1}{l}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Coverage}}  & \multicolumn{1}{c}{\textbf{Independence}}  & \multicolumn{1}{c}{\textbf{Joint}} \\ 
\hline
\multicolumn{4}{c}{\textbf{Real GDP}} \\ 
\hline
TVP-VAR-SV & 4.88^{\ast\ast} &  7.04^{\ast\ast\ast} &  11.92^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 16.93^{\ast\ast\ast} &  0.67 &  17.60^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 13.32^{\ast\ast\ast} &  0.66 &  13.98^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Inflation}} \\ 
\hline
TVP-VAR-SV & 0.02 &  3.64^{\ast} &  3.67 \\ 
GF-TVP-VAR-SV & 0.02 &  2.64 &  2.66 \\ 
CF-TVP-VAR-SV & 0.02 &  2.64 &  2.66 \\ 
\hline
\multicolumn{4}{c}{\textbf{FFR}} \\ 
\hline
TVP-VAR-SV & 16.93^{\ast\ast\ast} &  30.55^{\ast\ast\ast} &  47.49^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 13.32^{\ast\ast\ast} &  28.43^{\ast\ast\ast} &  41.76^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 18.88^{\ast\ast\ast} &  26.45^{\ast\ast\ast} &  45.33^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Credit Spread}} \\ 
\hline
TVP-VAR-SV & 4.88^{\ast\ast} &  17.62^{\ast\ast\ast} &  22.50^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 27.57^{\ast\ast\ast} &  39.78^{\ast\ast\ast} &  67.35^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 20.92^{\ast\ast\ast} &  47.14^{\ast\ast\ast} &  68.06^{\ast\ast\ast} \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: to be added}
\end{flushleft}
\end{table}


==> FcstTables/Table2InFevalCTestHorizon_1_Model_8_Prior_3_Lag_3_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[!t]\centering
\caption{$68\%$ Christoffersen Likelihood-Ratio Tests ($3$ Lags, horizon $8$)).}
\label{tab:InFevalCTestHorizon8Model1Prior3Lag3FcstNeval98SamplingMode1DifMode1FacMode1}
\begin{center}
\begin{tabular}{l *{3}{d{6.6}} }
\hline\hline
\multicolumn{1}{l}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Coverage}}  & \multicolumn{1}{c}{\textbf{Independence}}  & \multicolumn{1}{c}{\textbf{Joint}} \\ 
\hline
\multicolumn{4}{c}{\textbf{Real GDP}} \\ 
\hline
TVP-VAR-SV & 0.45 &  5.24^{\ast\ast} &  5.70^{\ast} \\ 
GF-TVP-VAR-SV & 0.88 &  6.63^{\ast\ast} &  7.51^{\ast\ast} \\ 
CF-TVP-VAR-SV & 0.88 &  3.98^{\ast\ast} &  4.85^{\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Inflation}} \\ 
\hline
TVP-VAR-SV & 0.51 &  6.27^{\ast\ast} &  6.78^{\ast\ast} \\ 
GF-TVP-VAR-SV & 1.71 &  5.64^{\ast\ast} &  7.35^{\ast\ast} \\ 
CF-TVP-VAR-SV & 1.02 &  2.06 &  3.08 \\ 
\hline
\multicolumn{4}{c}{\textbf{FFR}} \\ 
\hline
TVP-VAR-SV & 20.92^{\ast\ast\ast} &  54.35^{\ast\ast\ast} &  75.27^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 18.88^{\ast\ast\ast} &  46.10^{\ast\ast\ast} &  64.98^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 18.88^{\ast\ast\ast} &  53.27^{\ast\ast\ast} &  72.15^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Credit Spread}} \\ 
\hline
TVP-VAR-SV & 10.10^{\ast\ast\ast} &  54.43^{\ast\ast\ast} &  64.53^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 11.66^{\ast\ast\ast} &  55.95^{\ast\ast\ast} &  67.62^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 20.92^{\ast\ast\ast} &  43.33^{\ast\ast\ast} &  64.25^{\ast\ast\ast} \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: to be added}
\end{flushleft}
\end{table}


==> FcstTables/Table2InFevalCTestHorizon_1_Model_8_Prior_3_Lag_4_FcstNeval_98_SamplingMode_1_DifMode_1_FacMode_1.tex <==
\begin{table}[!t]\centering
\caption{$68\%$ Christoffersen Likelihood-Ratio Tests ($4$ Lags, horizon $8$)).}
\label{tab:InFevalCTestHorizon8Model1Prior3Lag4FcstNeval98SamplingMode1DifMode1FacMode1}
\begin{center}
\begin{tabular}{l *{3}{d{6.6}} }
\hline\hline
\multicolumn{1}{l}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Coverage}}  & \multicolumn{1}{c}{\textbf{Independence}}  & \multicolumn{1}{c}{\textbf{Joint}} \\ 
\hline
\multicolumn{4}{c}{\textbf{Real GDP}} \\ 
\hline
TVP-VAR-SV & 2.61 &  7.25^{\ast\ast\ast} &  9.86^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 1.71 &  5.64^{\ast\ast} &  7.35^{\ast\ast} \\ 
CF-TVP-VAR-SV & 2.61 &  3.46^{\ast} &  6.07^{\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Inflation}} \\ 
\hline
TVP-VAR-SV & 1.02 &  12.59^{\ast\ast\ast} &  13.61^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 1.02 &  4.30^{\ast\ast} &  5.31^{\ast} \\ 
CF-TVP-VAR-SV & 1.02 &  1.68 &  2.70 \\ 
\hline
\multicolumn{4}{c}{\textbf{FFR}} \\ 
\hline
TVP-VAR-SV & 13.32^{\ast\ast\ast} &  36.19^{\ast\ast\ast} &  49.52^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 23.05^{\ast\ast\ast} &  51.21^{\ast\ast\ast} &  74.26^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 27.57^{\ast\ast\ast} &  69.26^{\ast\ast\ast} &  96.82^{\ast\ast\ast} \\ 
\hline
\multicolumn{4}{c}{\textbf{Credit Spread}} \\ 
\hline
TVP-VAR-SV & 0.02 &  12.47^{\ast\ast\ast} &  12.48^{\ast\ast\ast} \\ 
GF-TVP-VAR-SV & 10.10^{\ast\ast\ast} &  42.47^{\ast\ast\ast} &  52.57^{\ast\ast\ast} \\ 
CF-TVP-VAR-SV & 16.93^{\ast\ast\ast} &  63.76^{\ast\ast\ast} &  80.70^{\ast\ast\ast} \\ 
\hline\hline
\end{tabular}
\end{center}
\begin{flushleft}
{\raggedright Notes: to be added}
\end{flushleft}
\end{table}


==> old_lemma2.tex <==
\mylemma{Subvector-Dynamics under TVP-VAR}{lemma_TVPVARsubvec}{
    Suppose $x_t \in \reals^n$ follows a TVP-VAR(1):
    \[
    x_t = \Phi_{0,t} + \Phi_{1,t}x_{t-1} + \Phi_{\varepsilon,t}\epsilon_t, \quad \epsilon_t \sim WN(0, I) \; .
    \]
    %
    Then any \(x^o_t \subseteq x_t\), $x^o_t \in \reals^k$ follows a TVP-VARMA(\(p',q'\)) with $p', q' \leq (n-k+1)$:
    \[
    x^o_t = \tilde{\Phi}_{0,t} + \sum_{l=1}^{p'} \tilde{\Phi}_{l,t}x^o_{t-l} + \sum_{k=1}^{q'} \tilde{\Theta}_{k,t}\tilde{\varepsilon}_{t-k} + \tilde{\Phi}_{\varepsilon,t}\tilde{\epsilon}_t \; , \quad \tilde{\epsilon}_t \sim WN(0, I) \; .
    \]
    If, more specifically, $x_t$ follows a RS-VAR(1) -- i.e. $\Phi_{0,t} = \Phi_{0}(s_t)$, $\Phi_{1,t}=\Phi_{1}(s_t)$ and $\Phi_{\varepsilon,t}=\Phi_{\varepsilon}(s_t)$  for $s_t \sim$ $n_s$-state Markov-chain with transition matrix $T$ --, 
    then $x^o_t$ follows a RS-VARMA (\(p',q'\)) with $p', q' \leq (n-k+1)$ and with $\tilde{\Phi}_{0,t} = \tilde{\Phi}_{0}(s_t)$, $\tilde{\Phi}_{l,t} = \tilde{\Phi}_{l}(s_t)$, $\tilde{\Theta}_{k,t} = \tilde{\Theta}_{k}(s_t)$ and $\tilde{\Phi}_{\varepsilon,t} = \tilde{\Phi}_{\varepsilon}(s_t)$.
}
\todo{Dalibor, please verify whether Normality and cont. diff. can be deleted}


\myproof{
    We consider a general time-variation.  
    The same argument goes through if the time-variation has a regime-switching nature.

    Partition \(x_t = (x^{o'}_t, x^{m'}_t)'\), where \(x^o_t \in \mathbb{R}^k\) are the retained variables and \(x^m_t \in \mathbb{R}^{n-k}\) are marginalized.
    Partition \(\Phi_{0,t}, \Phi_{1,t}, \Phi_{\varepsilon,t}\) conformably:
    \[
    \Phi_{0,t} =
    \begin{pmatrix}
    \Phi_{0,t}^o \\ \Phi_{0,t}^m
    \end{pmatrix}, \;
    \Phi_{1,t} =
    \begin{pmatrix}
    \Phi_{1,t}^{oo} & \Phi_{1,t}^{om} \\
    \Phi_{1,t}^{mo} & \Phi_{1,t}^{mm}
    \end{pmatrix}, \;
    \Phi_{\varepsilon,t} =
    \begin{pmatrix}
    \Phi_{\varepsilon,t}^{oo} & \Phi_{\varepsilon,t}^{om} \\
    \Phi_{\varepsilon,t}^{mo} & \Phi_{\varepsilon,t}^{mm}
    \end{pmatrix}.
    \]
    %
    The system for \(x^m_t\) is:
    \[
    x^m_t = \Phi_{0,t}^m + \Phi_{1,t}^{mo}x^o_{t-1} + \Phi_{1,t}^{mm}x^m_{t-1} + \Phi_{\varepsilon,t}^{mo}\epsilon_t^o + \Phi_{\varepsilon,t}^{mm}\epsilon_t^m.
    \]
    %
    Rewriting, we obtain:
    \[
    A_{mm,t}(L)x^m_t = \Phi_{0,t}^m + \Phi_{1,t}^{mo}x^o_{t-1} + \Phi_{\varepsilon,t}^{mo}\epsilon_t^o + \Phi_{\varepsilon,t}^{mm}\epsilon_t^m,
    \]
    where \(A_{mm,t}(L) = I_{n-k} - \Phi_{1,t}^{mm}L\). Assume \(A_{mm,t}(L)\) is nonsingular for all \(t\), i.e. \(\det(A_{mm,t}(L))\) is not identically zero, and that the inverse is well defined uniformly in \(t\). By Cramer's rule applied pointwise in \(t\),
    \[
    A_{mm,t}(L)^{-1} = \frac{\mathrm{adj}(A_{mm,t}(L))}{\det(A_{mm,t}(L))}.
    \]
    Here \(\mathrm{adj}(A_{mm,t}(L))\) is a matrix polynomial of degree \((n-k-1)\), and \(\det(A_{mm,t}(L))\) is a scalar polynomial of degree \((n-k)\). Thus, \(A_{mm,t}(L)^{-1}\) is a matrix rational function of degree at most \((n-k)\).
    
    Define
    \[
    \begin{aligned}
    C_{t}(L) &= A_{mm,t}(L)^{-1}\Phi_{0,t}^m, \\
    H_t(L) &= A_{mm,t}(L)^{-1}\Phi_{1,t}^{mo}, \\
    G^o_t(L) &= A_{mm,t}(L)^{-1}\Phi_{\varepsilon,t}^{mo}, \\
    G^m_{t}(L) &= A_{mm,t}(L)^{-1}\Phi_{\varepsilon,t}^{mm}.
    \end{aligned}
    \]
    %
    Shifting indices \(t \to t-1\), we obtain
    \[
    x^m_{t-1} = C_{t-1}(L) + H_{t-1}(L)x^o_{t-2} + G^o_{t-1}(L)\epsilon_{t-1}^o + G^m_{t-1}(L)\epsilon_{t-1}^m.
    \]
    %
    Substituting \(x^m_{t-1}\) into the first block equation for \(x^o_t\) yields:
    \begin{align*}
        x^o_t &= \Phi_{0,t}^o + \Phi_{1,t}^{oo}x^o_{t-1} + \Phi_{1,t}^{om}x^m_{t-1}  + \Phi_{\varepsilon,t}^{oo}\epsilon_t^o + \Phi_{\varepsilon,t}^{om}\epsilon_t^m \\
        &= \Phi_{0,t}^o + \Phi_{1,t}^{oo}x^o_{t-1} + \Phi_{1,t}^{om}C_{t-1}(L) + \Phi_{1,t}^{om}H_{t-1}(L)x^o_{t-2} \\
        & \quad + \Phi_{1,t}^{om}G^o_{t-1}(L)\epsilon_{t-1}^o + \Phi_{1,t}^{om}G^m_{t-1}(L)\epsilon_{t-1}^m + \Phi_{\varepsilon,t}^{oo}\epsilon_t^o + \Phi_{\varepsilon,t}^{om}\epsilon_t^m \\
        &= \tilde{\Phi}_{0,t} + \tilde{\Phi}_{t}(L)x^o_{t-1} + \tilde{\Theta}^o_t(L)\epsilon_t^o + \tilde{\Theta}^m_t(L)\epsilon_t^m \; ,
    \end{align*}
    where we define
    \[
    \begin{aligned}
        \tilde{\Phi}_{0,t} &= \Phi_{0,t}^o + \Phi_{1,t}^{om}C_{t-1}(L), \\
        \tilde{\Phi}_{t}(L) &= \Phi_{1,t}^{oo} + \Phi_{1,t}^{om}H_{t-1}(L)L, \\
        \tilde{\Theta}^o_t(L) &= \Phi_{1,t}^{om}G^o_{t-1}(L)L + \Phi_{\varepsilon,t}^{oo}, \\
        \tilde{\Theta}^m_t(L) &= \Phi_{1,t}^{om}G^m_{t-1}(L)L + \Phi_{\varepsilon,t}^{om}.
    \end{aligned}
    \]
    %
    Define the process $\tilde{\varepsilon}_t \sim WN(0,I)$, the matrix $\tilde{\Phi}_{\varepsilon,t}$ and the lag polynomial $\tilde{\Theta}_t(L)$ to be s.t.
    $$ \tilde{\Phi}_{\varepsilon,t}\tilde{\epsilon}_t + \tilde{\Theta}_t(L)\tilde{\epsilon}_t = \tilde{\Theta}^o_t(L)\epsilon_t^o + \tilde{\Theta}^m_t(L)\epsilon_t^m \; . $$
    %
    Overall, the reduced system for \(x^o_t\) becomes:
    \[
    x^o_t = \tilde{\Phi}_{0,t} + \tilde{\Phi}_{1,t}(L)x^o_{t-1} + \tilde{\Theta}_t(L)\tilde{\epsilon}_t + \tilde{\Phi}_{\varepsilon,t}\tilde{\epsilon}_t \; .
    \]
    %
    Hence \(x^o_t\) satisfies a finite-order TVP-VARMA(\(p',q'\)) representation with \(p',q' \leq (n-k+1)\).
    $\blacksquare$
}
\todo{shouldn't it be $n-k+1$ if there are these additional $L$'s in the definitions of Phis and Thetas?}
\todo{did I adjust the part pertaining to epsilon-tilde's correctly?}

\myremark{when \(q'=0\)}{
    The reduced system for \(x^o_t\) is a TVP-VAR(\(p'\)) process (i.e., \(q'=0\)) if and only if
    \[
    \Phi_{1,t}^{om} = 0 \ \text{and} \ \Phi_{\varepsilon,t}^{om} = 0,
    \]
    for all \(t\). In this case, the autoregressive degree satisfies \(p' \leq 1\), which is consistent with the general bound \(p' \leq (n-k)\).
}


\myremark{Wold decomposition}{
    If, in addition to the assumptions of Lemma 2, the time-varying lag polynomial \(A_t(L)=I-\Phi_{1,t}L\) is causal and uniformly invertible (i.e.\ \(\det (A_t(z))\neq 0\) for all \(|z|\le1\) and all \(t\)), then, by the results of \cite{karanasos2025unified}, the resulting TVP-VARMA\((p',q')\) process \(x^o_t\) admits a Wold--Cramér decomposition.
}


